Multi-Objective Model-based Reinforcement Learning for Infectious Disease Control

Severe infectious diseases such as the novel coronavirus (COVID-19) pose a huge threat to public health. Stringent control measures, such as school closures and stay-at-home orders, while having significant effects, also bring huge economic losses. In the face of an emerging infectious disease, a crucial question for policymakers is how to make the trade-off and implement the appropriate interventions timely given the huge uncertainty. In this work, we propose a Multi-Objective Model-based Reinforcement Learning framework to facilitate data-driven decision-making and minimize the overall long-term cost. Specifically, at each decision point, a Bayesian epidemiological model is first learned as the environment model, and then the proposed model-based multi-objective planning algorithm is applied to find a set of Pareto-optimal policies. This framework, combined with the prediction bands for each policy, provides a real-time decision support tool for policymakers. The application is demonstrated with the spread of COVID-19 in China.

==> Algorithms/Algo_SPSA.tex <==

\vspace{.2cm}
 \begin{algorithm}[!h]
% \SetAlgoLined
\KwData{tolerance $tol >0$, initial point $\vlam^1 \in E_1$,  step sizes $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}$, 
number of replications $M$,  direction distribution $\mathbb{G}$; 
other parameters $t_0, T, \mathcal{T}, c_l(\cdot)$,  
$\rho_{t_0}, X^I_{l, {t_0 - D}}, \{ X^R_{l,t}\}_{t = t_0 - D}^{t_0}, \{A_{l,t}\}_{t = t_0 - D}^{t_0 - 1}, w_{l,t_0}$ }

\textbf{Initialization:}
set $\delta = \infty$, $k = 1$, 
$X^{I,+}_{l, {t_0 - D}} = X^{I,-}_{l, {t_0 - D}} = X^I_{l, {t_0 - D}}$, $X^{R,+}_{l,t} = X^{R,-}_{l,t} = X^R_{l,t}$ for $ t \in \{t_0 - D, \dots, t_0\}$, 
and $A^{+}_{l,t} = A^{-}_{l,t} = A_{l,t}$ for $ t \in \{t_0 - D, \dots, t_0 -1\}$

\While{$\delta \ge tol$}{
    sample $\Delta_k \sim \mathbb{G}$; 
    set $\vlam^{k,+} = \vlam^k + \xi_k \Delta_k$ % more general?
    and $\vlam^{k,-} = \vlam^k - \xi_k \Delta_k$
    
    set $V_k^+ = V_k^- = 0$
    
    \For{$m=1,\dots,M$}{
        
        
        \For{$t'=t_0,\dots,T$}{
        sample $\vthe_{m, t'} \sim \rho_{t_0}$
        
            generate $S^{b,+}_{l, t'} =  MBS(\{ X^{R,+}_{l,t}\}_{t = t' - D}^{t'}$, 
              $\{A^{+}_{l,t}\}_{t = t' - D}^{t' - 1}, \rho_{t_0}, D)$

            choose action $A^+_{l,t'} = \pi(S^{b,+}_{l, t'}; \vlam_t^{k,+}) \mathbb{I}(t \in \mathcal{T}) + A^+_{l, t' - 1} \mathbb{I}(t \notin \mathcal{T})$
            
            sample $S^+_{l,t'+1} \sim  f(\cdot|S^+_{l,t'}, 
            A^+_{l,t'}; \vthe_{m, t'} )$ 
            and 
            $C^{A,+}_{l,{t'}} \sim c_l(A^+_{l,t'})$ 
            
            calculate  $Y^+_{l,{t'}} = 
            X^{S,+}_{l,t'} - X^{S,+}_{l,t'+1} + 
            \omega_{l,t_0} C^{A,+}_{l,{t'}}$

            generate $S^{b, -}_{l, t'} =  MBS(\{ X^{R,-}_{l,t}\}_{t = t' - D}^{t'}$, 
              $\{A^{-}_{l,t}\}_{t = t' - D}^{t' - 1}, \rho_{t_0}, D)$
              
            choose action $A^-_{l,t'} = \pi(S^{b, -}_{l, t'}; \vlam_{t_0}^{k,-}) \mathbb{I}(t \in \mathcal{T}) + A^-_{l, t' - 1} \mathbb{I}(t \notin \mathcal{T}) $
            
            sample $S^-_{l,t'+1} \sim  f(\cdot|S^-_{l,t'}, 
            A^-_{l,t'}; \vthe_{m, t'} )$ 
            and 
            $C^{A,-}_{l,{t'}} \sim c_l(A^-_{l,t'})$ 
            
            calculate  $Y^-_{l,{t'}} = 
            X^{S,-}_{l,t'} - X^{S,-}_{l,t'+1} + 
            \omega_{l,t_0} C^{A,-}_{l,{t'}}$
            

        }
        update $V_k^+ = V_k^+ + (T-t_0+1)^{-1}\sum_{t' = t_0}^{T} Y^+_{l,t'}$, 
        $V_k^- = V_k^- + (T-t_0+1)^{-1}\sum_{t' = t_0}^{T} Y^-_{l,t'}$
    }
    
    calculate $\bar{V}_k^+ = V_k^+ / M $, 
        $\bar{V}_k^- = V_k^- / M $
    
    Set $\vlam^{k+1} = \mathbb{P}_{E_k}(\vlam^{k} + \zeta_k (2\xi_k)^{-1} (\bar{V}_k^+ - \bar{V}_k^-) \Delta_k )$ 
    
    set $ k = k + 1$ and $\delta = ||\vlam^k - \vlam^{k-1}||/||\vlam^{k-1}||$ 
 }
 \KwResult{optimal policy parameters ${\boldsymbol{\lambda}}_{l,{t_0}} = {\boldsymbol{\lambda}}^k$ }  
 \caption{Simultaneous Perturbation Stochastic Approximation}\label{alg:SPSA}
\end{algorithm}
\vspace{.5cm}

%  and  recommended immediate action $\pi(S_{l,t_0}|\vlam_{l,{t_0}})$.

==> Archive/0_KDD_pre_Archive.tex <==


\section{Citations and Bibliographies}

The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

The bibliography is included in your source document with these two
commands, placed just before the \verb|\end{document}| command:
\begin{verbatim}
  \bibliographystyle{ACM-Reference-Format}
  \bibliography{bibfile}
\end{verbatim}
where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
suffix, of the \BibTeX\ file.

Citations and references are numbered by default. A small number of
ACM publications have citations and references formatted in the
``author year'' style; for these exceptions, please include this
command in the {\bfseries preamble} (before the command
``\verb|\begin{document}|'') of your \LaTeX\ source:
\begin{verbatim}
  \citestyle{acmauthoryear}
\end{verbatim}

  Some examples.  A paginated journal article \cite{Abril07}, an
  enumerated journal article \cite{Cohen07}, a reference to an entire
  issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
  monograph/whole book in a series (see 2a in spec. document)
  \cite{Harel79}, a divisible-book such as an anthology or compilation
  \cite{Editor00} followed by the same example, however we only output
  the series if the volume number is given \cite{Editor00a} (so
  Editor00a's series should NOT be present since it has no vol. no.),
  a chapter in a divisible book \cite{Spector90}, a chapter in a
  divisible book in a series \cite{Douglass98}, a multi-volume work as
  book \cite{Knuth97}, a couple of articles in a proceedings (of a
  conference, symposium, workshop for example) (paginated proceedings
  article) \cite{Andler79, Hagerup1993}, a proceedings article with
  all possible elements \cite{Smith10}, an example of an enumerated
  proceedings article \cite{VanGundy07}, an informally published work
  \cite{Harel78}, a couple of preprints \cite{Bornmann2019,
    AnzarootPBM14}, a doctoral dissertation \cite{Clarkson85}, a
  master's thesis: \cite{anisi03}, an online document / world wide web
  resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game
  (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05}
  and (Case 3) a patent \cite{JoeScientist001}, work accepted for
  publication \cite{rous08}, 'YYYYb'-test for prolific author
  \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
  contain 'duplicate' DOI and URLs (some SIAM articles)
  \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
  multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
  couple of citations with DOIs:
  \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
  citations: \cite{TUGInstmem, Thornburg01, CTANacmart}. Artifacts:
  \cite{R} and \cite{UMassCitations}.

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section{Appendices}


==> Archive/5_Broader_impact.tex <==
\section*{Ethics Statement}
We would like to emphasize that taking the economy as more  important than human lives is not a motivation or an outcome of this framework. 
On one hand, economic losses can also cause health damage to many people, probably not less than the direct damage from the disease; 
on the other hand, the estimated Pareto-optimal policies aim to help policymakers reduce the cost on one objective without sacrificing the other, as illustrated in Section \ref{sec:numerical_policy}. 

The framework is designed with the overall welfare of all people in mind. 
We acknowledge that the degree of interest loss for different groups may vary due to different choices among the Pareto-optimal policies, 
which is a tricky and unavoidable ethical question. 
For this purpose, 
an online interactive tool and an open-sourced software are under development to facilitate the real-time dissemination of results. 
Everybody is welcome to utilize these tools to have a better understanding of the current situation and participates in the discussion. 


% Two pages for references; optional ethics statement on these pages.
% Additionally, this year, we encourage authors to (optionally) write a statement about the potential ethical impact of their work, including its broad societal implications, both positive and negative.
% reviewers identify negative ethical concerns about a paper and it did not adequately address these concerns either in an ethics statement or in its main body.

% A widespread ethical concern during the outbreak of COVID-19 is .  


% \begin{figure}[t!]
% \centering		
% \includegraphics[width=.45\textwidth]{figures/action_plot.png} 	
% \caption{\hl{Move to supplement later. Not easy to read?}}
% \label{figure:action_plot}
% \end{figure}


% The validity of the proposed system depends on the prediction accuracy of the GSIR model as well as the modeling of the intervention costs. 
% A considerable error in either part may lead to a sub-optimal policy. 
% Fortunately, the online planning nature of the framework can mediate this issue, because the policymakers only need to select among a small set of actions every several days, and as long as the relative relationship between the prediction trajectories is reasonable, the system can recommend an appropriate action. 


% Nevertheless, it is the right action instead of accurate prediction itself that really matters. 


% Our method is generally applicable to infectious disease pandemics. 
% The direct users of this system is policymakers in each region, while everybody is 

% underreaction and overreaction, both having been witnessed. 
% too calm and objective


%%%%%%%%%%%%%%%%%%%%%%%% ARCHIVE %%%%%%%%%%%%%%%%%%%%%%%%
% Ethical Considerations in the example 
% Any text generation application that learns from data runs the risk of producing biased or offensive content reflective of the training data
% our work, which learns a language model from song lyrics, is no exception. 
% One approach that we implement is to moderate the words shown to our language model based on a list of keywords3; 
% a downside of this moderation is the potential for increased bias as a side effect of the content filter. 
% Recent work in modeling the intentions of vulgar expressions has shown promise for more nuanced profanity filtering or hate speech detection [12], and as these approaches improve, they present one path toward better automated moderation when working on text generation. 

% In addition to biased or offensive content, the other common ethical concern when working with material like lyrics is the potential for plagiarism. 
% In our setting, one of the reasons we choose to work with arbitrary audio inputs is to explicitly condition the language model with a strong signal which, intuitively, should make it difficult to copy from the training set; still, more work is needed to determine the extent to which the audio conditioning reduces plagiarism.

% For policymakers, however, it is the selection of the optimal control intervention in the face of uncertainty, rather than accuracy of model predictions, that is the measure of success that counts. 
% it is the selection of the optimal control interventions in the face of uncertainty that counts, and ultimately what they are judged on.


% Requirement: ethical aspects  and future societal consequences. (both positive and negative outcomes)
% \begin{enumerate}
%     \item who may benefit from this research and who may be put at disadvantage from this research
%     \item what are the consequences of failure of the system
%     \item whether the task/method leverages biases in the data
% \end{enumerate}


==> Archive/new_commands.tex <==
%%%%%%%%%%%%
\newcommand{\Mean}{{\mathbb{E}}}
\newcommand{\Var}{{\mathbb{VAR}}}
\newcommand{\Cov}{{\mathbb{COV}}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\lam}{\lambda}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
\newcommand{\vlam}{\boldsymbol{\lam}}
\newcommand{\vrho}{\boldsymbol{\rho}}
\newcommand{\hRI}{\widehat{RI}}
\newcommand{\vthe}{\boldsymbol{\theta}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mI}{\mathbb{I}}
\newcommand{\mA}{\mathcal{A}}
\renewcommand{\prob}{{\mathbb{P}}}
\newcommand{\mT}{\mathcal{T}}
\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\argmax}{arg\!max}
\renewcommand\not[1]{#1\xnot}

%%%%%%%%%%%%


==> Archive/packages.tex <==
\usepackage[ruled, vlined]{algorithm2e}
\setlength{\algomargin}{0em}

\usepackage{array}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{booktabs}

\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{soul}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{mathtools}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \userpackage{pdfpages}
% \usepackage{lineno}
% \usepackage{setspace}

% \usepackage[utf8]{inputenc}
% \usepackage[left=1.02in, right=1.02in, top=1.1in, bottom=1.05in]{geometry}
% \usepackage[font=small,labelfont=bf]{caption}
% \doublespacing
% \linenumbers


==> Archive/suppCOVID.tex <==
% \usepackage{amssymb}
\input{0_KDD_pre}
\usepackage{subcaption}

\usepackage{xr}
\makeatletter

\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\myexternaldocument{./0_MAIN}



\title{Supplement to ``Multi-Objective Model-based Reinforcement Learning for Infectious Disease Control"}

\begin{document}
\setcounter{section}{1}
	
\maketitle

\appendix 



\raggedbottom
\section{Posterior estimation of the GSIR model}\label{sec:MAP}
In this section, we introduce the derivation of the posteriors. 
% our prior family choices for $\vthe$ and
Recall our model (\ref{SIR}) is 
\begin{align*}
% \begin{split}
X^S_{l,t+1} &= X^S_{l,t} - e^S_{l,t}, e^S_{l,t} \sim  \text{Poisson}(\sum_{j=1}^J \beta_j \mathbb{I}(A_{l,t} = j) X^S_{l,t} \frac{X^I_{l,t}}{M_l}) ;\\ %   \hl{notation?}
X^R_{l,t+1 } &= X^R_{l,t} + e^R_{l,t}, e^R_{l,t} \sim \text{Binomial}(X^I_{l,t}, \gamma );\\
X^I_{l,t+1} &= M_l - X^S_{l,t+1} - X^R_{l,t+1 }, 
% \end{split}
\end{align*}
where the third equation is redundant. 
With data $\mathcal{D}_{t_0}$, the Markov property of the transition model reduces the estimation problem to $J + 1$ Bayesian generalized linear models with the identity link function. 
Specifically, let ${\Omega_{t_0,j}} = 
\{(t,l): 1 \leq t \leq t_0 - 1,
1 \leq l \leq N_{t}, 
A_{l,t} = j\}$ be the set of time-location pairs where action $j$ is taken, and let $\Omega_{t_0} = \{(t,l): 1 \leq t \leq t_0 - 1,
1 \leq l \leq N_{t}\}$. 
Assume $\{e^S_{l.t}, e^R_{l.t}|  1 \leq t \leq t_0 - 1,
1 \leq l \leq N_{t} \}$ are all independent, and then the likelihood function can be written as 
\begin{align*}
&\mathcal{L}( \vthe |\mathcal{D}_{t_0}) 
= \prod_{(t,l) \in \Omega_{t_0}} f_B(X^R_{l,t+1 } - X^R_{l,t}, X^I_{l,t}; \gamma)  \\
&\quad \times \prod_{j \in \{1, \dots, J\} } \prod_{(t,l) \in \Omega_{t_0,j}} f_P(
X^S_{l,t} - X^S_{l,t+1}; %\\ 
\sum_{j=1}^J \beta_j \mathbb{I}(A_{l,t} = j)  X^S_{l,t} X^I_{l,t} / M_l ), 
\end{align*} 
where $f_B(\cdot, \cdot; \cdot)$  is the density function of the Binomial distribution and $f_P(\cdot; \cdot)$ is that of the Poisson distribution. 
For simplicity, we consider the case that the parameter priors are independent with each other. 
For more general settings, approximate inference methods such as Markov Chain Monte Carlo can be used. 
For the recover rate $\gamma$, we use the Beta-Binomial conjugate pair and set its prior as $Beta(a_{R}, b_{R})$ with parameters 
$a_{R}$ and  $b_{R}$. 
For the infection rate $\beta_j$, $j = 1, \dots, J$, the Poisson-Gamma conjugate pair is used,
and we set the prior of $\beta_j$ as $ Beta(a_{S,j}, b_{S,j})$ with parameters 
$a_{S, j}$ and  $b_{S, j}$. 
By choosing these conjugate priors, the corresponding posterior distributions have explicit forms as $\gamma \mid \mathcal{D}_{t_0} \sim  Beta(a_{R}^* , b_{R}^*)$ 
and 
$\beta_j \mid \mathcal{D}_{t_0} \sim  Gamma(a_{S,j}^* , b_{S,j}^*)$, for $j = 1, \dots, J$
, where

\begin{equation*}
    \begin{aligned}
a_{S,j}^* &= a_{S,j} + \sum_{(t,l) \in \Omega_{t_0,j}}\left( {X_{l, t}^{S} - X_{l, t+1}^{S}}{} \right),\\
b_{S,j}^* &= b_{S,j}+ \sum_{(t,l) \in \Omega_{t_0,j}}  \frac{X_{l, t}^{S,j}X_{l, t+1}^{I}}{M_l}, \\
a_{R}^* &= a_{R} + \sum_{(t,l) \in \Omega_{t_0}} \left( {X_{l, t+1}^{R} - X_{l, t}^{R}} \right), \\ % (t,l)  because l \leq N_t depends on t --> t first then l or (l, t) location \sum_{l=1}^{N_{t_0}} \sum_{t=t_l}^{t_0-1}, where $t_l$ is the first day when region l has confirmed cases.
b_{R}^* &= b_{R}- \sum_{(t,l) \in \Omega_{t_0}}  \left( {X_{l, t+1}^{R} - X_{l, t}^{R}} \right) + \sum_{(t,l) \in \Omega_{t_0}} {X_{l, t}^{I}}.
\end{aligned}
\end{equation*}
\raggedbottom



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{More on the Policy Search Algorithms}
\subsection{Constrained simultaneous perturbation stochastic approximation}\label{sec:SPSA}

When $J$ is large, Algorithm \ref{alg:grid} in the main paper can be computationally expensive. 
In general, a variety of optimization algorithms, such as Bayesian optimization and heuristic optimization algorithms, can be applied here. 
As an example, we provide a constrained simultaneous perturbation stochastic approximation (SPSA) algorithm  \cite{sadegh1997constrained} here. 
%  for more general settings
It is described in Algorithm \ref{alg:SPSA}. 
In SPSA, we need to specify two step size sequences $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}$, which  should satisfy $\sum_{k = 1}^{\infty} \zeta_k = \infty, \sum_{k = 1}^{\infty} \zeta_k^2 < \infty$ and $\xi_k = o(1)$ as $k$ goes to infinity. %? not uniform?
% In our experiments, we use $\zeta_k = \zeta / k^{\tau}$ and $\xi_k = \xi/k$, where $\zeta, \xi$  and $\tau \in (0.5,1]$ are  tuning parameters. 
Unlike traditional SPSA, for each candidate parameter $\vlam_t^k$, we run $M$ replications of Monte Carlo instead of only once and use the average to approximate the expected average utility. 
This is because that, in our setting, the sampling is relatively cheap and the potential loss of a sub-optimal policy can be quite severe. 
The operator $\mathbb{P}_{E_k}$ is the orthogonal projection onto  $E_k$ and it ensures the feasibility of policy evaluation under the constraints. 
Following \cite{sadegh1997constrained}, we define $E_k = \{\vlam: \lam_J + \xi_k\sqrt{J - 1} \le \lam_M, \lam_i + \xi_k\sqrt{J - 1} \le \lam_{i + 1} , \forall i \in \{1,\dots,J-1\} \}$. 
The direction is sampled from a distribution $\mathbb{G}$ of dimension $J-2$. 
The convergence of SPSA is guaranteed by our choice of $\zeta_k$.
In implementations, 
warm start can be used by setting $\vlam^1 = \vlam_{t_0 - 1}$ to further reduce the computational burden and 
multi-start random initialization can also be employed to remedy the non-convexity. 
% \hl{needs update Ek. already done in the code}
% Denote the feasible parameter region as $E = \{\vlam: 0 \le \lam_2 \le \dots \le \lam_{J} \le \lam_M\}$. 


\input{Algorithms/Algo_SPSA.tex}


\subsection{Deep Q-learning}\label{sec:supp-DQN}
When the global optimality is preferred, we can choose a general policy class and apply cutting-edge RL algorithms to solve the planning problem. 
In Algorithm \ref{alg:DQN}, we modify the deep-Q learning algorithm to take into consideration the learned uncertainty on $\vthe$.  
% used in our experiment. 
More details abou the standard DQN can be found in \cite{mnih2015human}. 


\input{Algorithms/DQN}




\subsection{Computational complexity}\label{sec:complexity}

In this section, we discuss the computational complexity of our policy search algorithm. 
We first consider a general form of the grid search algorithm presented in Algorithm \ref{alg:grid}. 
Suppose we have $J$ action levels, and recall we have $J - 1$ policy parameters $\lam_2, \dots, \lam_J$. 
Let the step size for searching $\lam_j$ be $\xi_j$ and the corresponding upper search bound be $U_j$, for $j = 2, \dots, J$. 
Define $\eta = max_{j \in \{2, \dots, J\}} (U_j / \xi_j)$. 
Assume that for each candidate policy, we run $M$ replications of rollouts.  
Using similar iteration schedule with Algorithm \ref{alg:grid} in the main paepr,
the computational complexity is easy to calculate as $O(M T \eta^{J - 1})$, where $T$ is the horizon. 
Then it is straightforward to show that the computational complexity of Algorithm 1 is $O(MB T \eta^{J - 1} + BKT)$, where $B$ is the number of candidate weights and $K$ is the number of Monte Carlo replications. 
Due to the importance of a stable optimization algorithm in our application, we choose to use this grid search algorithm in our experiment and recommend a large $M$. 
This is feasible when $J$ is not large, for example, $3$ or $5$. 
However, because its complexity is of exponential order with respect to $J$, when there are many actions available, we should choose other optimization algorithms such as Algorithm \ref{alg:SPSA}, with a large $M$ to reduce the variance from Monte Carlo rollouts. 
The algorithm is embarrassingly parallel. 
For the DQN-based method, the complicity is $B$ times of that of the standard deep-Q learning algorithm. 

\subsection{Hyper-parameters}
In this section, we describe the hyper-parameters used in our experiments. 
For the grid search algorithm, the number of rollout replications is set as $M = 100$. 
We run the grid search algorithm from coarse grids to finer grids to save computational cost. 
The schedule is listed in Table \ref{table:para}. 
In generally, the larger the search spaces and the smaller the step sizes, the better the performance will be. 
In consideration of the importance of this application and the relatively lightweight computation, in real application, we can choose the search spaces as large enough and step size as small enough. 
% $\lambda_M$ is another upper bound which indicates that, no matter

For DQN, in our experiment, we use a dense network of 5 layers, with 32 nodes per layer, to model the Q-function. 
The activation function is picked as relu and the optimizer is set as Adam. 
The learning rate is fixed as 0.0002 and the parameter for epsilon-greedy is set as $\epsilon = 0.1$. 
% max_epoch = 100


% &   $\beta_3$ 
\begin{table*}[t!]
\centering
    \caption{Search space and step sizes for the grid search in each round. $\lam^i_1$ and $\lam^i_2$ are the output from the $i$-th round.}
    \label{table:para}
    \begin{tabular}{lllllll}
\toprule
  round & $u_2$  &  $u_3$    & $U_2$  & 
  $U_3$ &   $\xi_2$ &   $\xi_3$  \\
\midrule
1 & 0& 300& 50& 0& 100& 200 \\
2 &  max(0, $\lam^1_1$ - 50)&  $\lam^1_1$ + 50& 5& $\lam^1_2$ - 200& $\lam^1_2$ + 200& 20 \\
3 &  max(0, $\lam^2_1$ - 5)&  $\lam^2_1$ + 5& 1& $\lam^2_2$ - 20& $\lam^2_2$ + 20& 4 \\
4 &  max(0, $\lam^3_1$ - 1)&  $\lam^3_1$ + 1& 0.25& $\lam^3_2$ - 4& $\lam^3_2$ + 4& 1 \\
5 &  max(0, $\lam^4_1$ - 0.25)&  $\lam^4_1$ + 0.25& 0.01& $\lam^4_2$ - 1& $\lam^4_2$ + 1& 0.2 \\
\bottomrule
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Details of the numerical experiments}

% In this section, we provide mores details of Section \ref{sec:numerical} and addtional numerical results. 

\subsection{More on the China COVID-19 dataset and hyper-parameters}\label{sec:supp-data}

We obtain the counts of cumulative confirmed cases $O_{l,t}^I$ from  \cite{China_Data} with irregular records imputed by the average of their neighbors.
The original mobility data collected from the online plateform Baidu Qianxi\footnote{http://qianxi.baidu.com} includes ${m_{l,t}^{20}}$, the mobility of people in city $l$ on day $t$ in  2020, and ${m_{l,t}^{19}}$, the value for the same date in 2019, aligned by the lunar calendar.  
We define $r_{l,t}=1- m_{l,t}^{20}/m_{l,t}^{19}$ to 
measure the  ratio of human mobility loss due to $A_{l,t}$. 
The fitted distributions for the intervention cost function are $C_2 \sim \mathcal{N}(0.368, 0.239^2)$ and 
$C_3 \sim \mathcal{N}(0.484, 0.181^2)$.
% C_3 rather than C_2
As for the action data, we collect the date ranges for different control measures claimed by Chinese local governments. 
The date ranges for action $1$ and $2$ as well as the starting dates for action $3$ are collected from \cite{wiki:action}. 
The ending dates for action $3$ are manually collected from the local government websites or their social media accounts. 
These data sources are all in Chinese. 
We use the estimates for SARS \cite{mkhatshwa2010modeling} to set the priors for the disease features, specifically, we set $\gamma \sim Beta(178.89, 2000)$ and $ \beta_1 \sim Gamma(517.41, 2000)$.
As for $\beta_2$ and $\beta_3$, similar with the assumptions in \cite{ferguson2020impact}, we assume the two measures reduce the infection rate by $80\%$ and $90\%$ respectively, and therefore use $\beta_2 \sim Gamma(103.48 , 2000)$ and $ \beta_3 \sim Gamma(51.74, 2000)$. 


% Since $X_{l,t}^R$ should be monotonically non-decreasing with respect to $t$ and there are some records violating this quality, we have substituted the peculiar records with mean values of their neighbors. 
% Figure \ref{fig:cost} shows the boxplot of the mobility loss ratio for different actions. 




\subsection{Validation of the simulation environment}\label{sec:supp_val}

We apply a leave-one-out cross-validation procedure to show that our simulation environment is close to the real data generation process. 
Specifically, for $l = 1, \dots, 6$, we follow the steps: 
\begin{enumerate}
    \item estimate the environmental parameter $\vthe$ as $\hat{\vthe}_l$, using all data  until day $61$ of cities in $\{1, \dots, 6\} \setminus \{l\}$.
    % day 10 = [2020-01-24]
    % day 61 = [2020-03-15]
    % day 120 = [2020-05-13]
    \item for city $l$, based on $\hat{\vthe}_l$, we predict its counts of the cumulative infected cases from day $12$ to day $120$, following the observed actions in the data. Denote the estimate for day $120$ as $\hat{X}^R_{120, l}.$ 
    % , t=10, 11,\cdots, 120$.
    \item calculate the approximation error by $\epsilon_{l} = |\hat{X}^R_{120, l} - O^I_{120,l}| / O^I_{120,l}$, where $O^I_{120,l}$ is the observed cumulative infected count for city $l$ until day $120$. 
\end{enumerate}

The average error ratio $\sum_{l = 1}^6 \epsilon_{l} / 6 = 0.18$  indicates that the environment is a relatively valid proxy for the real data generation process, 
and supports the fairness of our comparison with the behaviour policy. 

\subsection{Statistical significance of the policy evaluation results}

In Figure \ref{figure:Pareto} in the main paper, we compare  our algorithm with the other competing policies by 
the average costs following each policy. 
To examine the statistical significance of our results, we report the corresponding $95\%$ confidence interval for each average value in Figure \ref{figure:Paretosquare}. 
We can observe that our findings in Section \ref{sec:policy} are  statistically significant. 
The variance for the DQN-based method is slightly larger due to the limited computational resources, and we expect it will become stabler with more computation. 
Results for the other experiments are similar. 

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{figures/more_final_val.png}
% 	\caption{Validation result with the least RMSE, where $\mathcal{L}_i=\{$Beijing, Guangzhou, Shanghai$\}$ and $\mathcal{L}'_i=\{$Hefei, Nanjing, Tianjin$\}.$}\label{fig:cv3}
% \end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{figures/main_with_DQN_sd.png} 
% Figure1_supp_factor10
\caption{Cumulative epidemiological cost and economic cost  following different policies, averaged over $100$ replications. The closer to the left bottom corner, the better. With the shaded areas indicating the 95$\%$ confidence regions.}
\label{figure:Paretosquare}
\end{figure}

\subsection{Sample policies displayed in the demo}
In Figure \ref{fig:pareto_demo}, we apply the policy search algorithm in the threshold-based policy class, and zoom in to analyze three Pareto-optimal policies. 
Here, we give their policy parameters to provide more details. 
For policy A, B, and C, their $\vlam$ is $(0,0)^T$, $(0.26,  420)^T$, and $(245, 573)^T$, respectively. 
This explains their behaviour: policy A is a strict one and assigns level 3 whenever the algorithm believes there is any infectious individual; 
policy B is milder, and it typically imposes the level-2 action unless the spread is quite severe; policy C is much more loose. 


\section{Sensitivity analysis}\label{sec: supp-robust}

\subsection{Robustness against model missepcification}\label{sec: supp-robust-analysis}
In this section, we investigate the robustness of the proposed framework against potential model missepcification. 
We use a generalized Susceptible-Exposed-Infected-Removal model (SEIR) model instead of the GSIR model as the data generation model, and conduct a simulation study similar with the one in Section \ref{sec:numerical_policy}. 
% with the setting kept the same
The standard SEIR model is another commonly used compartmental model, which adds one additional exposed compartment to the SIR model. 
See Figure \ref{figure:SEIR} for an illustration and refer to \cite{tang2020review} for a detailed introduction. 

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{figures/SEIR.png} 
\caption{A diagram for the standard SEIR model.}
\label{figure:SEIR}
\end{figure}

We generalize the SEIR model in a similar with as the GSIR model, by including the action effects into consideration to set the infection rate $\beta$. The transition from the susceptible compartment to the exposed compartment is assumed to follow a binomial distribution with parameter $\alpha$. 
According to \cite{yang2020modified}, we set the incubation rate $\alpha$ as $1/7$. 
The other parameters are kept the same with Section \ref{sec:numerical_policy}. 
Since the exposed compartment is typically latent,  the number of individuals in this compartments on the beginning date can not be set based on the real data as the other compartments. 
For experiment purpose, we set the number to be the same with the number in the infectious compartment. 

The results are presented in Figure \ref{figure:Pareto_SEIR}. 
As expected, compared with results under the GSIR model, the performance of the  proposed method under this setting slightly deteriorates. 
However, in generally, the method still over-performs the other fixed policies, and also provides more options with a clear trade-off.  



\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{figures/SEIR_with_DQN.png} 
\caption{Simulated results when the true data generation model is the generalized SEIR model. Cumulative epidemiological cost and economic cost  following different policies, averaged over $100$ replications.}
\label{figure:Pareto_SEIR}
\end{figure}


\subsection{Hyper-parameter sensitivity analysis}\label{sec:sensitivity}
Our framework requires selecting several hyper-parameters according to domain knowledge, and our choices in the experiments largely follow the practice in the early period of the COVID-19 outbreak and are listed in Section \ref{sec:supp-data}. 
On one hand, at the beginning of an pandemic we have to rely on some priors to make decision; and on the other hand, in this section we use numerical experiments to evaluate the robustness of our algorithm to these hyper-parameters. 
The setting is kept the same with Section \ref{sec:numerical_policy}, except for that we only run 25 replications for the proposed algorithm to save computation. 
We present results for the threshold-based policy class. 
Results for the DQN-based methods are similar and omitted. 

In Figure \ref{figure:robust_lag}, we report the results with $D = 7, 8, 9, 10, 11$. 
It can be seen that, although the results varies a little, the algorithm generally still outperform the competing policies, and our findings in Section \ref{sec:numerical_policy} still hold. 

% \begin{figure}[h!]
% \centering
% \includegraphics[width=.45\textwidth]{figures/robust_lag.png} 
% \caption{Robust analysis results for the hyper-parameter $D$.}
% \label{figure:robust_lag}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width=.45\textwidth]{figures/robust_effect.png} 
% \caption{Robust analysis results for the hyper-parameter $\mu_1$ and $\mu_2$.}
% \label{figure:robust_effect}
% \end{figure}


\begin{figure*}[t]
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=.8\textwidth]{figures/robust_lag.png} 
\caption{Robust analysis results for the hyper-parameter $D$.}
\label{figure:robust_lag}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=.8\textwidth]{figures/robust_effect.png} 
\caption{Robust analysis results for the hyper-parameter $\mu_1$ and $\mu_2$.}
\label{figure:robust_effect}
\end{subfigure}
\caption{Hyper-parameter sensitivity analysis}
\label{fig:sensitivity}
\end{figure*}



Similarly, we report the robustness analysis results for the treatment effects $\mu_2$ and $\mu_3$ In Figure \ref{figure:robust_effect}. 
Recall that we define $\mu_j = \beta_j / \beta_1$ and use it to set the prior for $\beta_i$. 
In our experiment, we use $\mu_2 = 0.2$ and $\mu_3 = 0.1$. 
In this analysis, we present results for $\{(\mu_2, \mu_3): \mu_3 \in \{0.05, 0.1, 0.15, 0.2\}
, \mu_2 - \mu_3 \in \{0.05, 0.1, 0.15, 0.2\} )\}$. 
These prior parameters turn out have little important in the long run, because their effects get washed out quickly by the observed data. 
The findings for the other prior parameters are similar. 

\break

\bibliography{bib}
\bibliographystyle{plain}
	
\end{document}


==> Archive/supp_sty.tex <==

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
% \usepackage{neurips_2020}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2020}

% to avoid loading the natbib package, add option nonatbib:
% \usepackage{Mis/neurips_2020}
\usepackage{Mis/aaai21}
\input{Mis/packages}


\usepackage{amsmath}
\usepackage{graphicx}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{algorithm,algpseudocode,enumerate}
\usepackage{bm}
\usepackage{hyperref}       % hyperlinks
\usepackage{xr-hyper}
% \usepackage{pdfpages}
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\myexternaldocument{0_MAIN}
\newtheorem{lemma}{Lemma}[section]

==> COVID_KDD (Camara Ready) [Arxiv]/0_Intro_abs.tex <==
\begin{abstract}
Severe infectious diseases such as the novel coronavirus (COVID-19) pose a huge threat to public health. 
Stringent control measures, such as school closures and stay-at-home orders, while having significant effects, also bring huge economic losses. 
In the face of an emerging infectious disease, 
a crucial question for policymakers is how to make the trade-off and implement the appropriate interventions timely given the huge uncertainty. 
In this work, we propose a Multi-Objective Model-based Reinforcement Learning framework to facilitate data-driven decision-making and minimize the overall long-term cost. 
Specifically, at each decision point, a Bayesian epidemiological model is first learned as the environment model, and then the proposed model-based multi-objective planning algorithm is applied to find a set of Pareto-optimal policies. 
This framework, combined with the prediction bands for each policy,  provides a real-time decision support tool for policymakers. 
The application is demonstrated with the spread of COVID-19 in China. 
\end{abstract}
% off-policy, greedy, infectious disease control, , MDP, online, 
% balance  long-term epidemiological and  economic costs.
 % travel restrictions
 


==> COVID_KDD (Camara Ready) [Arxiv]/1_Intro.tex <==

\section{Introduction}\label{sec:intro}
The novel coronavirus (COVID-19) has spread rapidly and 
posed a tremendous threat to the global public health \cite{world2020coronavirus}. 
Among the efforts to contain its spread, 
several strict control measures, including school closures and workplace shutdowns, 
have shown high effectiveness \cite{anderson2020will}. 
Nevertheless, these measures bring enormous costs to economies and other public welfare aspects at the same time \cite{eichenbaum2020macroeconomics}. 
For example, an unprecedented unemployment rate in the United States partially caused by some COVID-19 control measures is anticipated by economists \cite{gangopadhyaya2020unemployment}. 
In the face of an emerging infectious disease, 
there are usually multiple objectives conflicting with each other, and either overreaction or under-reaction may result in a substantial unnecessary loss. 
A crucial question for policymakers all around the world is 
\textit{how to make the trade-off and intervene at the right time and in the right amount to minimize the overall long-term cost to the citizens.}

This work is motivated by the ongoing COVID-19 pandemic, where it is witnessed that the decision-making can be impeded by huge intervention costs, great uncertainty on the infectious ability of the disease and the effectiveness of different interventions, and various concerns over the long-term impacts. 
This paper aims to provide a real-time data-driven decision support framework for policymakers. 
We formalize the problem under the multi-objective Markov decision process (MOMDP) framework and integrate epidemiology models, statistical methods, and reinforcement learning algorithms to address this problem. 







\input{1_Intro_contribution}
\input{1_Intro_related_work}




==> COVID_KDD (Camara Ready) [Arxiv]/1_Intro_contribution.tex <==
\textbf{Contribution.  }
Our contributions are multi-fold. 
First, as our transition model, 
we generalize the celebrated Susceptible-Infected-Removal (SIR) model \cite{kermack1927contribution} to allow simultaneous estimation of the infectious ability of this disease and evaluation for the effectiveness of different control measures, in an online fashion. 
There is a vast literature on modeling and prediction for infectious diseases; see \cite{keeling2011modeling} for an overview. 
Among these works, compartmental models such as the SIR model are widely used; see, e.g., \cite{song2020epidemiological} and \cite{sun2020tracking} for applications to COVID-19.  
During an outbreak, the knowledge about the infectious ability and the effectiveness of interventions usually change a lot,
and a quantitative decision-making support tool should utilize the update-to-date information timely. % incorporate
However, none of these works considers online parameter updating and intervention effect estimation at the same time. 
% hence is not applicable to decision-making in an urgent situation such as the COVID-19 outbreak. 
We aim to achieve this goal via an online Bayesian framework. 

Second, we propose a novel online planning framework to assist policymakers in making decisions that minimize the overall long-term cost. 
In real applications, policymakers generally group different interventions into several ordered levels with increasing strictness and choose among them subsequently (e.g., in the U.S. \cite{korevaar2020quantifying} and New Zealand \cite{wilson2020pandemic}). 
This paper will focus on selecting among such a set of ordinal actions. 
% The current work would assist governments’ decision-makings among these levels with the economic costs in mind.
Specifically, at each decision point, on the ground of the estimated generalized SIR model, 
we propose a model-based planning algorithm to learn the optimal intervention policy, for each given weight between the two competing objectives, i.e., minimizing the epidemiological cost and the economic cost. 
Both interpretable policy classes and complex black-box classes are considered. 
We then extend the algorithm to obtain a representative set of Pareto-optimal policies, i.e., policies that cannot be improved for one objective without sacrificing another.
This framework, combined with the prediction bands for each policy, achieves the goal of supporting multi-objective decision-making. 
Compared with the huge literature on infectious disease modeling and prediction, 
the optimal decision-making problem is far less studied. 
Most works either focus on the evaluation of several fixed interventions 
\cite{tildesley2006optimal, ferguson2020impact, hellewell2020feasibility} 
or study the optimal control problem with a deterministic model \cite{ledzewicz2011optimal, elhia2013optimal}. 
None of these works allows sequential decision making with online updated parameter estimation,
which enables selecting the appropriate intervention according to the current state and available data. 
In addition, the long-term effect is particularly important in this application due to the spread nature of the pandemic. 
Reinforcement learning (RL) is particularly suitable for these purposes, while its application in infectious disease control is relatively new to the literature.
The existing works are mainly concerned with problems caused by limited resources \cite{probert2018real, laber2018optimal}, such as vaccine limitations in controlling seasonal flu. 
In contrast, we focus on another aspect, the multi-objective problem caused by the huge costs of stringent control measures. 
This approach provides us with a clearer view of the trade-off. 
To our knowledge, this is the first work on applications of multi-objective RL to infectious disease control. 

Third, we present an application of our method to control the outbreak of COVID-19 as an example, which is important in its own right. 
Our proposed framework is generally applicable to pandemic controls. 
To investigate the robustness, applications to other diseases and several sensitivity analyses are also studied. 



==> COVID_KDD (Camara Ready) [Arxiv]/1_Intro_related_work.tex <==
\textbf{Related work.  } 
In addition to the aforementioned literature on infectious disease-related modeling, our methodology also belongs to the field of reinforcement learning. 
Our problem is closely related to the line of research on MOMDPs (see \cite{roijers2013survey} or \cite{liu2014multiobjective} for a survey), which studies problems with multiple competing objectives. 
When the weights between objectives are unknown, the literature focuses on obtaining the whole class of Pareto-optimal policies approximately \cite{castelletti2012tree, barrett2008learning, parisi2017manifold, pirotta2015multi}. 
Because of the online planning nature in our case, it suffices to adopt a simpler approach, by performing multiple runs of policy search over a representative set of weights \cite{van2013scalarized, natarajan2005dynamic}. 

Besides, RL algorithms are commonly classified as model-based methods (e.g., MBVE \cite{feinberg2018model}, MCTS \cite{browne2012survey}, etc.), which directly learn a model of the system dynamics, and model-free methods (e.g., fitted-Q iteration \cite{riedmiller2005neural}, deep-Q network \cite{mnih2015human}, 
actor-critic \cite{konda2000actor}, etc.), which do not. 
In the case of emerging infectious disease control, on one hand, the algorithm needs to generalize to unseen transitions (e.g., the end of the epidemic), where the model-free approach is typically not applicable \cite{van2019use}; 
on the other hand, some epidemiological models have demonstrated satisfactory prediction power. 
Therefore, the model-based approach is adopted in this paper. 

Finally, we note that some efforts have been made in the literature to study the control policy for COVID-19 \cite{alvarez2020simple,piguillem2020optimal,eftekhari2020markovian}. 
As discussed above, these works did not consider the multi-objective problem. 
In addition, they focus on solving a one-time planning problem to decide all future actions instead of providing a real-time decision-making framework. 
RL algorithms have also been applied to learn the 
vaccine distribution strategy \cite{awasthi2020vacsim} or to control mobility \cite{song2020reinforced}. 

% but assigned a fixed price for each life to scalarize the objective

% Alvarez: planning, stat life
% umich.
% Multi-objective. 
% Real-time decision-making

% Atkeson (2020) computes the projected paths of the disease and evaluates its eco- nomic impact.
% Eichenbaum, Rebelo, and Trabandtz (2020) construct what they call a SIR-macro model with endogenous consumption and labor supply.
% 1. Estimation. Planning. 
% 2. Assume a fixed price for each 
% 3. A unique angle to 
% How to plan for the future actions. 
% Online planning
% As noted above, 
% Dynamic, Multi-objective 



% Finally, we take the policy-based approach \cite{williams1992simple, silver2014deterministic, lillicrap2015continuous} instead of the value-based approach \cite{riedmiller2005neural, mnih2015human} to facilitate interpretability, which is vital in our application. 
% Specifically, we first propose an interpretable policy class, and then run direct policy search by applying optimization algorithms to maximize the value function approximated via Monte Carlo rollouts.  
% Refer to \cite{gosavi2015simulation} for a review of the applications of simulation-based optimization in RL. 


% This paper differs with  existing works about decision-making in epidemiology in two aspects: 

% Specifically, a learning and planning schedule is adopted:  


==> COVID_KDD (Camara Ready) [Arxiv]/2_pre_MDP.tex <==
\subsection{Multi-objective Markov decision process}\label{sec:pre_MOMDP}
A Markov decision process (MDP) \cite{puterman2014markov} is a sequential decision making model which can be represented by a tuple $\langle \mathcal{S}, \mathcal{A}, c, f \rangle$, where 
$\mathcal{S}$ is the state space, 
$\mathcal{A}$ is the action space, 
$c : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is the expected cost function, 
and $f : \mathcal{S}^2 \times \mathcal{A}  \rightarrow \mathbb{R}$ is a Markov transition kernel. 
Throughout the paper we use the term \textit{cost} instead of \textit{reward}. 
A multi-objective MDP (MOMDP) is an extension of the MDP model when there are several competing objectives. 
An MOMDP can be represented as a tuple $\langle \mathcal{S}, \mathcal{A}, \mathbf{c}, f \rangle$, where the other components are defined as above and $\mathbf{c} = (c^1, \dots, c^K)^T$ is a vector of $K$ cost functions for $K$ different objectives, respectively. 

In this paper, we consider the finite horizon setting with a pre-specified horizon $T$. 
The horizon can simply be selected as a large enough number without loss of generality, since the costs we consider will be close to zero after the disease being controlled. 
Besides, we focus on deterministic policies for realistic consideration, 
since to assign an intervention by randomization may not be feasible. 
For a deterministic policy $\pi$, we define its $k$-th value function at time $t_0$ as $V_{k, t_0}^\pi(s) =  \mathbb{E}_{\pi}( \sum_{t=t_0}^{T} 
c^k(S_t, A_t)|S_{t_0} = s)$, where $\mathbb{E}_{\pi}$ denotes the expectation assuming $A_{t} = \pi(S_t)$ for every $t \ge t_0$. 

In the MDP setting, the objective is typically to find an optimal policy $\pi^*$ that minimizes the expected cumulative cost among a policy class $\mathcal{F}$.
However, in an MOMDP, there may not be a single policy that minimizes all costs. 
Instead, we consider the set of Pareto-optimal policies with linear preference functions $\Pi_{t_0} = \{\pi \in \mathcal{F} : \exists \boldsymbol{\omega} \in \boldsymbol{\Omega} \; \text{s.t.} \; 
\boldsymbol{\omega}^T \boldsymbol{V}_{t_0}^{\pi}(s) \le \boldsymbol{\omega}^T \boldsymbol{V}_{t_0}^{\pi'}(s), 
\forall \pi' \in \mathcal{F}, s \in \mathcal{S} \}$, 
where $\boldsymbol{\Omega} = \{\boldsymbol{\omega} \in \mathbb{R}_+^{K}: \boldsymbol{\omega}^T \boldsymbol{1} = 1\}$ and $\boldsymbol{V}_{t_0}^{\pi} = (V_{1, t_0}^\pi, \dots, V_{K, t_0}^\pi)^T$. 
A policy is called \textit{Pareto-optimal} if it can not be improved for one objective without sacrificing the others. 
The dependency on $t_0$ is to be consistent with the online planning setting considered in this paper. 


==> COVID_KDD (Camara Ready) [Arxiv]/2_pre_SIR.tex <==
\subsection{The Susceptible-Infected-Removal model}\label{sec:SIR}
The compartmental models are, arguably, the most popular choices in epidemiology modeling \cite{tang2020review}. 
These models will divide the population into different compartments with labels, and model the transitions of people between these compartments to describe the mechanism of infectious diseases spread. 

Among these models, the Susceptible-Infected-Removal (SIR) model is one of the most widely applied models \cite{brauer2008compartmental}. 
Suppose at time $t$, the infectious disease is spread within $N_t$ regions. Denote the total population of the $l$-th region as $M_l$, for $l=1,\dots, N_t$. 
With the SIR model, we divide the total population into three groups: the individuals who can infect others, who have been removed from the infection system, and  who have not been infected and are still susceptible. 
Denote the count for each group in region $l$ at time $t$ as $X^I_{l,t}$, $X^R_{l,t}$, and $X^S_{l,t} = M_l - X^I_{l,t} - X^R_{l,t}$, respectively. 
We will discuss how to construct these variables using surveillance data   in Section \ref{sec:delayed}. 
The standard deterministic SIR model can then be written as 
a system of difference equations: 
% \begin{alignat*}{1}
%     X^S_{l,t+1} &= X^S_{l,t} - \beta X^S_{l,t} X^I_{l,t}/ M_l;\\[-1pt]
%     X^I_{l,t+1} &= X^I_{l,t} + \beta X^S_{l,t} X^I_{l,t}/ M_l
%     -  \gamma X^I_{l,t};\\[-1pt]
%     X^R_{l,t+1} &= X^R_{l,t} +  \gamma X^I_{l,t}, 
% \end{alignat*}
\begin{align*}
    X^S_{l,t+1} &= X^S_{l,t} - \beta X^S_{l,t} X^I_{l,t}/ M_l;\\
    X^I_{l,t+1} &= X^I_{l,t} + \beta X^S_{l,t} X^I_{l,t}/ M_l
    -  \gamma X^I_{l,t};\\
    X^R_{l,t+1} &= X^R_{l,t} +  \gamma X^I_{l,t}, 
\end{align*}
where $\beta$ and $\gamma$ are constants representing the infection and removal rate, respectively. 
A diagram for the SIR model is given in Figure \ref{fig:SIR_diagram}. 


\begin{figure}[!h]
\centering
\includegraphics[width=.5\textwidth]{figures/SIR.png}
\caption{The infectious disease spread mechanism described by the SIR model.}
\label{fig:SIR_diagram}
\end{figure}


==> COVID_KDD (Camara Ready) [Arxiv]/3_GSIR.tex <==
\subsection{The generalized SIR model}\label{sec:GSIR}
In this work, we aim to modify the SIR model as our transition model. 
We note that some other compartmental models such as the SEIR model  \cite{brauer2008compartmental} can also fit in our framework. 
However, with limited data and knowledge in the face of an emerging infectious disease, the SIR model has been found to be a robust choice \cite{roda2020difficult}. 

There are two limitations with the standard SIR model. 
First, the infection rate heavily depends on the control measure being taken. 
As discussed in Section \ref{sec:intro}, in this paper we focus on an ordinal set of actions  $\mathcal{A} = \{1, 2, \dots, J\}$, with level $1$ standing for no official measures. 
Second, a stochastic model with proper distribution assumptions is required to fit real data with randomness. 
Motivated by the discussions above, we propose the generalized SIR (GSIR) model and use it as our \textbf{transition model}:

\begin{align}
\label{SIR}
\begin{split}
X^S_{l,t+1} &= X^S_{l,t} - e^S_{l,t}, \;\;  e^S_{l,t} \sim  \text{Poisson}(\sum_{j=1}^J \beta_j \mathbb{I}(A_{l,t} = j) X^S_{l,t} \frac{X^I_{l,t}}{M_l} ) ;\\
X^R_{l,t+1 } &= X^R_{l,t} + e^R_{l,t}, \;\;  e^R_{l,t} \sim \text{Binomial}(X^I_{l,t}, \gamma );\\
X^I_{l,t+1} &= M_l - X^S_{l,t+1} - X^R_{l,t+1 }, 
\end{split}
\end{align}
where $\mathbb{I}(\cdot)$ is the indicator function, 
$A_{l,t}$ is the action taken by region $l$ at time $t$, 
and  $\beta_j$ denotes the infection rate under action $j$. 
The choice of the Poisson and the Binomial distribution is popular in the literature \citep{held2019handbook}, and is motivated by their probabilistic
implications. 
We assume $\beta_1 \ge \beta_2 \ge \dots \ge \beta_J \ge 0$ to represent the increasing effectiveness. 
The estimation of $\vthe = (\gamma, \beta_1, \dots, \beta_J)^T$ is deferred to Section \ref{sec:sir_est}. 



%%%%%%%%%%%%%%%%%% Delayed %%%%%%%%%%%%%%%%%%
% Introduce it later？ OK?
% We assume individuals in $X^R_t$ have already been well isolated and thus removed from the infectious system. 
% Although $X^I_t$ can not be observable directly, we will find a good proxy for it in Section \ref{sec:delayed}. 
%%%%%%%%%%%%%%%%%% Delayed %%%%%%%%%%%%%%%%%%

% in region $l$ at time $t$, traditionally treated as constants.
% However, in reality, the transition model is not homogeneous across both the spatial and temporal dimension. 
% For example, in the control of COVID-19, 
% it is witnessed that $\beta_{l,t}$ depends heavily on the control measure adopted, and $\gamma_{l,t}$ on the testing ability. 

% we focus on a discrete set of ordered actions which are encoded as $A_{l,t} \in \{1, 2, \dots, J\}$, with the effect assumption $\beta_1 > \beta_2 > \dots > \beta_J \ge 0$. Here, $A_{l,t} = 1$ represents no specific measure, and action $j$ is more strict and effective than action $i$ when $j > i$. % generalize? % cost



% First, the control and testing ability may be heterogeneous among different regions.
% \hl{To characterize this point, we introduce two pre-specified functions $f_1(\cdot)$ and $f_2(\cdot)$  to incorporate heterogeneities depending on the region-specific static features $X_l$. }


==> COVID_KDD (Camara Ready) [Arxiv]/3_MDP.tex <==
\subsection{Sequential decision making}\label{sec:MDP}
In this work, we focus on the intervention decision of each region: 
in the model estimation (learning) step, data from several similar regions are 
aggregated to share information and mitigate the issue that data is typically noisy, scarce, and single-episode in a pandemic; 
while in the decision-making (planning) step, each region chooses its own action.
% in infectious disease control 



\textbf{MOMDP definition.  }
The intervention decision-making problem can be naturally formalized as an MOMDP.
For each region $l$, 
at each decision point $t$, according to the estimated transition model, the current  \textbf{state} $S_{l,t} = (X^S_{l,t}, X^I_{l,t}, X^R_{l,t})^T$, and their judgment, 
the policymakers determine a \textbf{policy} $\pi_{l,t}$ with the objective of  minimizing the overall long-term cost, 
and  choose the \textbf{action} $A_{l,t}$ to implement according to the policy. 
This action, assuming being effectively executed, will affect the infection rate during $(t, t+1]$ and hence the conditional distribution of $S_{l,t+1}$. 
Let $f(\cdot|\cdot, \cdot; \vthe)$ be the 
conditional density for $S_{l, t+1}$ given $S_{l,t}$ and $A_{l,t}$ in model (\ref{SIR}). 
In this work, we consider two cost variables, the \textbf{epidemiological cost} $C^E_{l,t}$ and the \textbf{action cost} $C^A_{l,t}$. 
$C^E_{l,t}$ can be naturally chosen as the number of new infections $X^S_{l,t} - X^S_{l,t+1}$. 
Let $C^A_{l,t} = c_{l}(Z_{l,t}, A_{l,t}, Z_{l,t+1}) \in \mathbb{R}^+$ for a time-varying  variable  $Z_{l,t}$ and a stochastic function $c_l$. 
Both $c_l$ and  $Z_{l,t}$ should be chosen by domain experts. 
For example, with $Z_{l,t}$ representing the unemployment rate, $C^A_{l,t} = Z_{l,t + 1} - Z_{l,t}$ can represent its change due to $A_{l,t}$. 
% In general, we should also include $Z_{l,t}$ in the state and model its transition.
Since the modeling for action cost and its transition is a separate question, for simplicity, 
we focus on the case that $C^A_{l,t} = c_l(A_{l,t})$ for a pre-specified  stochastic function $c_l(\cdot)$ in this paper. 
$c_l(\cdot)$ is set to be region-specific to incorporate local features, such as the economic conditions. 
With a given weight $\omega_{l,t} \in \mathbb{R}^+$, the \textbf{overall cost} $C_{l,t}$ is then defined as $C^E_{l,t} + \omega_{l,t} C^A_{l,t}$.
The expected cost functions can then be derived from these definitions, and for decision-making purposes, the overall cost is equivalent with the weighted cost defined in Section  \ref{sec:pre_MOMDP} when $K = 2$. 



\textbf{Online planning.  } 
The RL problem considered in this paper is an \textit{online planning}, or sometimes called \textit{planning at decision time} problem \cite{sutton2018reinforcement}, which  focuses on selecting an action for the current state with collected environment information. 
We consider a sequence of decision points $\mathcal{T} \subset \{1, \dots, T\}$ to reduce the action switch cost in real applications. 
At time $t_0 \notin \mathcal{T}$, the region keeps the same action with time $t_0 - 1$. 
At time $t_0 \in  \mathcal{T}$, 
the policymakers choose an action according to the decision-making workflow displayed in Figure \ref{fig:diagram}. 

We summarize Figure \ref{fig:diagram} as follows. 
For each region $l$, at the decision point $t_0$, 
we first estimate the posterior  of $\vthe$ as  $\rho_{t_0}$, using accumulated data $\mathcal{D}_{t_0} {=} \{S_{l,t}, A_{l,t}\}_{1 \le l \le N_{t_0}, 1 \le t \le t_0 - 1} \cup \{S_{l,t_0}\}_{1 \le l \le N_{t_0}}$ and priors selected with domain knowledge. 
Next, the policymakers choose the trade-off weight  $\omega_{l, t_0}$, 
learn a deterministic policy $\hat{\pi}_{l, t_0}(\cdot; \omega_{l, t_0})$ by planning, and implement $A_{l,t_0} {=} \hat{\pi}_{l, t_0}(S_{l,t_0}; \omega_{l, t_0})$. 
% c_l
Formally, we solve the following optimization problem to obtain $\hat{\pi}_{l, t_0}(\cdot; \omega_{l, t_0})$:
% We focus on the greedy  because it may not be realistic to 
% do exploration or accept a stochastic policy under such a serious situation. 
\vspace{-.3cm}
\begin{align}
\hat{\pi}_{l, t_0}(\cdot; \omega_{l, t_0}) = \argmin_{\pi \in \mathcal{F}} \mathbb{E}_{\pi, \rho_{t_0}}( \sum_{t=t_0}^{T}(  C^E_{l,t} + \omega_{l, t_0}  C^A_{l,t})), 
\label{fomular:objective}
\end{align}
where  $\mathbb{E}_{\pi, \rho_{t_0}}$ denotes the expectation assuming 
$C^A_{l,t} \sim c_l(A_{l,t})$, 
$\prob(S_{l, t+1} = s_{l, t+1} |S_{l,t}\! =  s_{l,t}, A_{l,t}\! = a_{l,t} ) \!= f(s_{l, t+1} |s_{l,t}, a_{l,t}; \vthe)$ with $\vthe  \,{\sim}\, \rho_{t_0}$, and 
$A_{l,t} \!= \pi(S_{l,t})\mathbb{I}(t \in \mathcal{T}) \!+ A_{l,t-1} \mathbb{I}(t \notin \mathcal{T})$, 
for every $t {\ge} t_0$. 

The Bayesian approach is preferred because 
(i) we need to make decisions before accumulating sufficient data,  and typically there is important domain knowledge available, and 
(ii) in this important application, the estimation uncertainty should be taken into consideration in decision-making.  
The specification of $\mathcal{F}$ and the policy search algorithms for solving (\ref{fomular:objective}) will be discussed in Section \ref{sec:policy}. 

% and the optimality in the remaining paper is discussed within $\mathcal{F}$. 



==> COVID_KDD (Camara Ready) [Arxiv]/3_Pareto.tex <==

\subsection{Multiple objectives and Pareto-optimal policies}\label{sec:Pareto}
In the discussion above, 
we assume the tradeoff weight $\omega_{l, t_0}$ is easily specified at each decision point $t_0$. 
This is feasible when the two objectives share the same unit, for example, when $C^A_{l,t}$ represents the damage to public health due to economic losses. 
In general settings, properly choosing the weight is not easy and sometimes unrealistic.
Therefore, we aim to assemble a decision support tool that provides a comprehensive picture of the future possibilities associated with different weight choices and hence makes the multi-objective decision-making feasible.

Solving the whole set of Pareto-optimal policies is typically challenging. 
While in our online planning setting, at each decision point $t_0$, 
we only need to make a one-time decision among a few available actions. 
For this purpose, it suffices to solve problem (\ref{fomular:objective}) for a representative set of weights $\{\omega_b\}_{b=1}^B$ to find the corresponding Pareto-optimal policies, and then apply Monte Carlo simulation to obtain the corresponding prediction bands for the potential costs following each policy. 
The policymakers can then compare all these possible options, select among them, and hence choose the action $A_{l, t_0}$. 
With this module, our framework is an \textit{user-in-the-loop} tool. 
A demo of some information presented to the users is displayed in Figure \ref{fig:pareto_demo}. 
We summarize this tool in Algorithm \ref{alg:tool}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/Demo_Pareto.png}
  \caption{Expected cumulative costs for different policies, with the corresponding recommended immediate actions indicated by the shape. 
  }
\end{subfigure}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{.2cm}
\begin{subfigure}{.23\textwidth}
  \centering
  \vspace{-.6cm}
  \includegraphics[width=.9\linewidth]{figures/demo_cost_XR.png}
  \caption{ 
  Mean trajectory and prediction bands of the predicted cumulative epidemiological costs. 
  }
\end{subfigure}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{.2cm}
\begin{subfigure}{.23\textwidth}
  \centering
  \vspace{-.6cm}
  \includegraphics[width=.9\linewidth]{figures/demo_cost_A.png}
  \caption{
    Mean trajectory and prediction bands of the predicted cumulative action costs. 
  }
\end{subfigure}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{.2cm}
\begin{subfigure}{.23\textwidth}
%   \vspace{-.6cm}
  \centering
  \includegraphics[width=.9\linewidth]{figures/demo_action.png}
  \caption{
  Mean trajectory of the predicted recommended actions. 
  Levels are averaged over replications and hence may not be integers. 
  }
\end{subfigure}%

\caption{A demo of some information presented to the users. 
Results are computed for Beijing, China on 02/10/2020. 
% decision point 
The proposed method is run under the experiment setting introduced in Section \ref{sec:numerical}, where we consider three levels of actions. 
For three sample policies, we plot the predicted behaviour of them in subplot (b)-(d). 
Prediction results are aggregated over $1000$ replications. 
According to subplot (d), policies A and B  can be interpreted as the suppression and mitigation policy studied in  \cite{ferguson2020impact}, and  policy C is close to the periodic lockdown policy suggested in the literature \cite{bin2020post, karin2020cyclic}.  
% The learned policy parameters are given and discussed in the supplement.
% To choose the current weight and action. 
}
\label{fig:pareto_demo}
\end{figure*}
% The  are plotted in subplot (a), 
% For two representative policies, we plot the mean actions, the , and the prediction bands for the  costs in subplot (b), (c), (d), respectively. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\input{Algorithms/Algo_Pareto.tex}

	
% (within the policy family) 

% In those cases, we are interested in a set of trade-off solutions that balance the objectives. More precisely, we want to obtain the set of best trade-off solutions, i.e., the set of solutions that Pareto dominate all the other solutions but are mutually incomparable.
% This means that it is not obvious how to define the weights in order to get a good coverage of the Pareto front of policies.

% and provides the policymakers with
% The decision makers only need to choose among three levels?
% It accords with the normal decision-making process and 
% MORE INTRODUCTION HERE!
% use notation for this set to save space?


% \hl{In the discussion above,} we assume the tradeoff weight $\omega_{l,t}$ is easily specified at each decision point, for instance, when $C^A_{l,t}$ and $C^E_{l,t}$ share comparable units. However, choosing the weight properly is not easy and sometimes unrealistic. 
% Thus, we present a decision support tool that provides a comprehensive picture of future possibilities associated with different weights.


% \hl{discuss typical MORL solution?}
% \hat{\pi}_{l, t_0}(\cdot; \omega_{l, t_0})
% Instead, we consider the set of Pareto-optimal policies with linear preference functions $\Pi_{t_0} = \{\pi \in \mathcal{F} : \exists \boldsymbol{\omega} \in \Omega \; \text{s.t.} \; 
% \boldsymbol{\omega}^T V_{t_0}^{\pi}(s) \le \boldsymbol{\omega}^T V_{t_0}^{\pi'}(s), 
% \forall \pi' \in \mathcal{F}, s \in \mathcal{S} \}$, 
% where $\boldsymbol{\Omega} = \{\boldsymbol{\omega} \in \mathbb{R}_+^{K}: \boldsymbol{\omega}^T \boldsymbol{1} = 1\}$. 
% A Pareto-optimal policy is defined as a policy that can not be improved for one objective without sacrificing the others. 
% The dependency on $t_0$ is to be consistent with the online planning problem considered in this paper. 

% For each weight $\omega_{l,t}$, the policy search algorithm for the  generates one Pareto-optimal policy. 


==> COVID_KDD (Camara Ready) [Arxiv]/4_SIR_est.tex <==
\subsection{Estimation of the transition model}\label{sec:sir_est}
At each time $t_0 \in \mT$, we need to first obtain the posterior of $\vthe$ in the transition model (\ref{SIR}). 
Notice that the last equation in (\ref{SIR}) is  redundant under the constraint $X^S_{l,t} + X^I_{l,t} + X^R_{l,t} = M_l$ for all $t$. 
With data $\mathcal{D}_{t_0}$, 
the Markov property reduces the estimation problem to $J + 1$  Bayesian generalized linear models with the identity link function. 
By choosing the priors as the conjugate priors, the posterior distributions have explicit forms. 
Specifically, let $\gamma \sim Beta(a_{R}, b_{R})$ with parameters $(a_{R}, b_{R})$, and  let $\beta_j \sim Beta(a_{S,j}, b_{S,j})$ with parameters $(a_{S, j}, b_{S, j})$, for $j = 1, \dots, J$. 
Under the assumption that these priors are independent, we have 
$\gamma \mid \mathcal{D}_{t_0} \sim  Beta(a_{R}^* , b_{R}^*)$ and 
$\beta_j \mid \mathcal{D}_{t_0} \sim  Gamma(a_{S,j}^* , b_{S,j}^*)$, for $j = 1, \dots, J$ , where
\begin{align*}
a_{S,j}^* &= a_{S,j} + \smashoperator{\sum_{(t,l) \in \Omega_{t_0,j}}} \left( {X_{l, t}^{S} - X_{l, t+1}^{S}}{} \right),
b_{S,j}^* = b_{S,j}+ \smashoperator{\sum_{(t,l) \in \Omega_{t_0,j}}}  \frac{X_{l, t}^{S}X_{l, t+1}^{I}}{M_l}, \\
a_{R}^* &= a_{R} + \smashoperator{\sum_{(t,l) \in \Omega_{t_0}}} \left( {X_{l, t+1}^{R} - X_{l, t}^{R}} \right), %\\ % (t,l)  because l \leq N_t depends on t --> t first then l or (l, t) location \sum_{l=1}^{N_{t_0}} \sum_{t=t_l}^{t_0-1}, where $t_l$ is the first day when region l has confirmed cases.
b_{R}^* = b_{R}- \smashoperator{\sum_{(t,l) \in \Omega_{t_0}}}  \left( {X_{l, t+1}^{R} - X_{l, t}^{R}} \right) + \smashoperator{\sum_{(t,l) \in \Omega_{t_0}}} {X_{l, t}^{I}}, 
\end{align*}
where  
${\Omega_{t_0,j}} {=}
\{(t,l) : 1 {\leq} t {\leq} t_0 {-} 1,
1 {\leq} l {\leq} N_{t}, 
A_{l,t} {=} j\}$ is the set of time-location pairs where action $j$ is taken, and $\Omega_{t_0} {=} \bigcup_j \Omega_{t_0,j}$. 
% The derivations are postponed to Section \ref{sec:MAP} in the supplement. 

% To save space, we postpone the derivations to Section \ref{sec:MAP} in the supplement. 
Below, we introduce a way to specify the prior parameters: 
(i) $\beta_1$ and $\gamma$ are both features of this disease without any interventions, and we can first set their priors with the estimates of similar diseases, and update them when additional biochemical findings are available;
(ii) for $j \geq 2$, $\beta_j$  indicates the infection rate under action level $j$. 
Suppose we have a reasonable estimate of the intervention effect $u_j= \beta_j / \beta_1$ as $\hat{u}_j$ and that of $\beta_1$ as $ \hat{\beta}_1$, then the prior of $\beta_j$ can be set as a distribution with expectation $\hat{u}_j \hat{\beta}_1$. 




==> COVID_KDD (Camara Ready) [Arxiv]/4_delayed.tex <==
\subsection{State construction}\label{sec:delayed}
In this section, we discuss the construction of state variables with surveillance data. 
The data usually available to policymakers is the cumulative count of confirmed cases until time $t$, denoted as $O^I_{l,t}$. 
% with a serious infectious disease, 
Unlike the infectious disease spread in nature, the individuals counted in $O^I_{l,t}$ generally either have been confirmed and isolated, or have recovered or died. 
Therefore, these individuals can be regarded as those removed from the infection system, and it is natural to set $X^R_{l,t}$ as $O^I_{l,t}$ \cite{yang2020sir}.  

Besides, for infectious diseases, there is typically a time delay between being infectious and getting isolated, the length of which is treated as a random variable with expectation $D$. 
Therefore, the count of the infectious $X^I_{l,t}$ is usually not immediately observable at time $t$, but will be gradually identified in the following days. 
Following the existing works on infectious disease modelling \cite{zhang2005compartmental, chen2020data}, 
we treat this issue as a delayed observation problem and use $O^I_{l,t + D} - O^I_{l,t}$, the new confirmed cases during $(t, t+D]$, as a proxy for $X^I_{l,t}$. 
In the planning step, following the literature on delayed MDPs \cite{walsh2009learning}, we apply Algorithm \ref{alg:MBS} (Model-based Simulation, MBS) to generate a proxy state, and then choose the action according to it. 
We note that although this issue is not obvious in prediction, it is unavoidable in  decision-making because $A_{l,t}$ works directly on $X^I_{l,t}$. 
% It also reminds us that our control decisions should be based on the latent state instead of only the confirmed cases. 
The performance of such an approximation is supported by the theoretical analysis in \cite{walsh2009learning} and 
the experiments in Section \ref{sec:numerical}. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%% Before renaming %%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Delayed observations}\label{sec:delayed}
% For infectious diseases, there is typically a time delay between being infectious and getting isolated, the length of which is treated as a random variable with expectation $D$. 
% Therefore, the count of the infectious $X^I_{l,t}$ is usually not immediately observable at time $t$, but will be gradually identified in the following days. 
% Following the existing works on infectious disease modelling \cite{zhang2005compartmental, chen2020data}, 
% we treat this issue as a delayed observation problem and consider the following approach. 
% Let $O^I_{l,t}$ be the count of cumulative confirmed cases until time $t$, then statistically, $O^I_{l,t + D} - O^I_{l,t}$, the new confirmed cases during $(t, t+D]$, can be a good proxy for $X^I_{l,t}$. 
% Similarly, $O^I_{l,t}$ can represent the number of individuals removed from the epidemiology system. 
% % and we assume the individuals counted in $O_{l,t}$ have been well isolated.
% In the planning step, following the literature on delayed MDPs \cite{walsh2009learning}, we apply Algorithm \ref{alg:MBS} (Model-based Simulation, MBS) to generate a belief state, and then choose the action according to it. 
% We note that although this issue is not obvious in prediction, it is unavoidable in  decision-making because $A_{l,t}$ works directly on $X^I_{l,t}$. It also reminds us that our control decisions should be based on the latent state instead of only the confirmed cases. 
% \hl{Mention the good numerical performance? (the performance of such an approximation is examined using numerical experiments in Section )} \ref{sec:numerical}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hence, we treat this issue as a delayed observation problem and construct the state variables as $X^I_{l,t} = O^I_{l,t+D} - O^I_{l,t}$ and $X^R_{l,t} =  O^I_{l,t}$ in the estimation step, 

% % Previous
% In the discussion above, the state $S_{l,t}$ is assumed to be observable at time $t$. 
% However, the SIR model is originally designed to describe the underlying dynamics of infectious diseases, % as a mathematical model
% and how to align its variables with data  requires additional attention. 
% The surveillance data usually available to policymakers includes the cumulative count of confirmed cases until time $t$, denoted as $O^I_{l,t}$. 
% We assume the individuals counted in $O^I_{l,t}$ have been  isolated. 
% However, $X^I_{l,t}$ counts the infectious who will be affected by the intervention and thus have not been isolated, hence $X^I_{l,t}$ is generally not observable at time $t$. 
% Inspired by existing works on SARS \cite{zhang2005compartmental} and COVID-19 \cite{chen2020data}, we treat this issue as a delayed observation problem and propose the following solution. 
% For infectious diseases, there is usually a delay between being infectious and getting isolated. 
% We treat its length as a random variable with expectation $D$.
% For example, according to \cite{sun2020tracking} and references therein, $D$ is reported to be between 8.36 and 9.1 days for COVID-19 cases in China, and the standard deviation of this duration is relatively small. 
% % mean; put in the data descriptin part
% Hence, although $X^I_{l,t}$ is not observable on day $t$, 
% it will gradually reveal in the following days. 
% Statistically, we treat $O^I_{l,t + D} - O^I_{l,t}$, the new confirmed cases during $(t, t+D]$, as a proxy for $X^I_{l,t}$.
% % , the already infected but not yet confirmed cases. 
% Similarly, we set $X^R_{l,t} = O^I_{l,t}$ to represent the individuals removed from the epidemiology system. They either have been confirmed and thus isolated, or have recovered or died. 
% % For this reason, the relationship  should  hold statistically. 
% % the validity of this procedure is evaluated in Section 4.2
% % simply apply the procedure
% %  as prepossessing
% With the observations above, 
% following the literature on delayed MDPs \cite{walsh2009learning}, 
% we construct the state variables as $X^I_{l,t} = O^I_{l,t+D} - O^I_{l,t}$ and $X^R_{l,t} =  O^I_{l,t}$, and use them in the estimation step. 
% In the planning step, we apply  Algorithm \ref{alg:MBS} (Model-based Simulation, MBS) to generate a belief state, and then choose action according to it. 
% We note that although this issue is not obvious in prediction, it is unavoidable in  decision-making because $A_{l,t}$ works directly on $X^I_{l,t}$. It also reminds us that our control decisions should be based on the latent state instead of only the confirmed cases.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Algorithms/Algo_MBS.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% For infectious diseases, there is usually a time delay between being infectious and getting isolated, the length of which is treated as a random variable with expectation $D$. Thus, the state variable $X^I_{l,t}$ defined in Section \ref{sec:SIR} as the count of the population who are infectious is generally not observable at time $t$. However, inspired by existing works on SARS \cite{zhang2005compartmental} and COVID-19 \cite{chen2020data}, $O^I_{l,t}$ $O^I_{l,t + D} - O^I_{l,t}$, the new confirmed cases during $(t, t+D]$ is a good proxy for $X^I_{l,t}$, where $O^I_{l,t}$ is the cumulative count of confirmed cases until time $t$ and is generally observable. Similarly, we use $O^I_{l,t}$ as a proxy for $X^R_{l,t}$ to represent the individuals removed from the epidemiology system.

% Hence, we treat this issue as a delayed observation problem and construct the state variables as $X^I_{l,t} = O^I_{l,t+D} - O^I_{l,t}$ and $X^R_{l,t} =  O^I_{l,t}$ in the estimation step, following the literature on delayed MDPs \cite{walsh2009learning}.
% In the planning step, we apply  Algorithm \ref{alg:MBS} (Model-based Simulation, MBS) to generate a belief state, and then according to which choose a corresponding action. 
% We note that although this issue is not obvious in prediction, it is unavoidable in  decision-making because $A_{l,t}$ works directly on $X^I_{l,t}$. It also reminds us that our control decisions should be based on the latent state instead of only the confirmed cases.


%%%%%%%%%%%%%%%%%%%

% mention delay [at least for action; we did not mention it]
% The augmented approach: verses us [if using all available past information?][and not interpretable and stable?]
% use examples to mention previous action is important now

% Therefore, either $O^I_{l,t}$ or $O^I_{l,t} - O^R_{l, t}$ is not equal to $X^I_{l,t}$, which counts the individuals who are able to transmit the virus onward and generally have not been identified yet. 

% Delayed observations


==> COVID_KDD (Camara Ready) [Arxiv]/4_policy_search.tex <==

\subsection{Policy search}\label{sec:policy}
At each decision point $t_0 \in \mathcal{T}$, for each region $l$ and a given weight $\omega_{l, t_0}$, we need to learn the optimal policy $\hat{\pi}_{l, t_0}(\cdot; \omega_{l, t_0}) \in \mathcal{F}$ by solving the model-based planning problem (\ref{fomular:objective}). 
We introduce two types of policy classes and the corresponding planning  algorithms, with emphasis on either the interpretability or the global optimality.  

% $\mathcal{F}$ is supposed to be a general and interpretable , 
% since interpretability is of great importance in this application. 
% \textbf{Interpretability-oriented policy class.} 
\textbf{Interpretable policy class.  } 
In applications of infectious disease control, the interpretability of the policy is typically important. 
In this case, we need to restrict our attention to an interpretable parametric policy class. 
As an illustration, in this work, we consider the following observations from the pandemic control decision-making process in real life: 
(i) the decision should be based on the spread severity, which we interpret as $X^I_{l,t}$, the number of infectious individuals; 
(ii) the policy should also be based on the current estimate of disease features $\rho_{t_0}$, the current state $S_{l, t_0}$, the trade-off weight $\omega_{l,t_0}$, and the potential cost $c_l(\cdot)$, which have all been incorporated in the objective function of (\ref{fomular:objective}); 
(iii) the more serious the situation, the more stringent the intervention should be. 
Motivated by these observations, we focus on the 
threshold-based policy class: 
\begin{equation}\label{eqn: policy_class_thre}
\begin{split}
 \mathcal{F} = \{\pi : \pi(S_{l,t}; \vlam) = \sum_{j=1}^{J} j \mathbb{I}(\lam_j \le X^I_{l,t} < \lam_{j+1}), \\ 0 = \lam_1 \le \lam_2 \le \dots \le \lam_{J + 1} = M_l, \lam_J \le \lam_M
    \}, 
\end{split}
\end{equation}
where $\vlam = (\lam_2,\dots, \lam_{J})^T$.
Notice that $X^I_{l,t}$ is generally a number much smaller than the population $M_l$, 
we introduce the pre-specified tolerance parameter $\lam_{M} \in (0,M_l)$ to reduce the computational cost by deleting unrealistic policies. 

Given  a specified policy class, problem (\ref{fomular:objective}) can be then solved via  rollout-based direct policy search. 
Direct policy search algorithms \cite{gosavi2015simulation} generally apply optimization algorithms to maximize the value function approximated via Monte Carlo rollouts. 
For class (\ref{eqn: policy_class_thre}), since the state transition and the action cost are both computationally affordable to sample, 
when $J$ is not large,  we can simply apply the grid search algorithm, which is  robust and safe in such an important application. 
% to efficiently and robustly find the optimal policy. 
The example for $J = 3$, which is the case in our experiment, is described in Algorithm \ref{alg:grid} in Appendix \ref{sec:pseudo_code}. 
When $J$ is large, many other optimization algorithms such as the simultaneous perturbation stochastic approximation algorithm  \cite{sadegh1997constrained} can be used.  
Alternatively, one can apply the deterministic policy gradient \citep{silver2014deterministic} or actor-critic 
\citep{lillicrap2015continuous} with the learned environment model as a simulator. 
% and a simultaneous perturbation stochastic approximation algorithm  \cite{sadegh1997constrained} is provided in Section \ref{sec:SPSA} of the supplement. 
% The computational complexity of our algorithm is discussed in Section \ref{sec:complexity} of the supplement. 



% \textbf{Optimality-oriented policy class.} 
\textbf{Black-box policy class.  } 
% \textbf{Neural network-based policy class.} 
If the interpretability can be traded off for global optimality, a more complex policy class can be considered. 
Since the action set is discrete, multiple planning algorithms in the literature are applicable, such as Monte carlo tree search with state aggregation \cite{hostetler2014state}. 
As an example, in this work, we focus on the policy class $\mathcal{F}$ induced by a class of deep-Q value network (DQN) \cite{mnih2015human} with an augmented state space $\mathcal{S} \times \{1, 2, \dots, T\}$. 
Specifically, to take into consideration the learned model uncertainty $\rho_{t_0}$, we define the Q-function of policy $\pi$ as $Q^\pi_{l, t_0}((s,t'), a; \omega_{l, t_0}) = \mathbb{E}_{\pi, \rho_{t_0}}( \sum_{t=t'}^{T}(  C^E_{l,t} + \omega_{l, t_0}  C^A_{l,t}))$, and then apply value iteration with epsilon-greedy exploration to learn the optimal value function as $\hat{Q}^*_{l, t_0}(\cdot, \cdot; \omega_{l, t_0})$. 
The corresponding policy is the induced greedy policy. 
More details can be found in Appendix \ref{sec:pseudo_code}. 
% of the supplement. 
% To save space, we defer the details to Section \ref{sec:supp-DQN} of the supplement. 
% will be $\hat{\pi}_{l, t_0}(s; \omega_{l, t_0}) = argmin_a \hat{Q}^*_{l, t_0}((s,t), a; \omega_{l, t_0})$. 






==> COVID_KDD (Camara Ready) [Arxiv]/5_Pareto.tex <==


\subsection{Evaluation of the Pareto-optimal policies}\label{sec:numerical_policy}
In this section, we conduct simulation experiments to compare the performance of our proposed method  with several competing policies on curbing the spread of COVID-19. 
Specifically, for the six cities, we start from day $12$ together, 
% with $(M_l - O^I_{l,21}, O^I_{l,21} - O^I_{l,12}, O^I_{l,12} )^T$ as the initial state for city $l$, 
and follow the actions recommended by a specific policy until day $120$, with the cumulative costs recorded. 
The state transitions are generated from the GSIR model with  $\mathbb{E}(\rho_{61})$ as the parameter, and the observations before day $12$ are kept the same with the real data. 
% and the variables $\{O^I_{l,t}\}_{1 \le t \le 12}, \{A_{l,t}\}_{1 \le t \le 11}, X_l$ as well as $M_l$ are the same with the real dataset, for $l \in \{1, \dots, 6\}$. 
This design is to mimic a real infectious disease control following some  specified policy or algorithm. 
Although this is a simulation study, we still investigated the validity of $\mathbb{E}(\rho_{61})$ as the environment parameter for fair comparison with the observed costs in the real data. 
Its validity is supported by the cross-validation results in Appendix \ref{sec:supp_val}. % in the supplement. 
It also partially supports that these regions are similar. 
% The validity of $\mathbb{E}(\rho_{61})$ as the environment parameter is supported by cross-validation in Section \ref{sec:supp_val} in the supplement.  

% fixed
We compare our algorithm with several  expert policies that are motivated by real life observations and commonly considered in the literature \cite{merl2009statistical, lin2010optimal, ludkovski2010optimal}. 
Specifically, the comparisons are made among the following policies: 
\begin{enumerate}
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}%
    \item Our proposed Pareto-optimal policies $\pi_k$ for $k \in \{-2, 0, \dots, 6\}$:  we fix the weight as $e^{k}/10$ across all cities and time, and follow the workflow proposed in Section \ref{sec:MDP}. $\mathcal{T}$ is set as every seven days. 
    We consider both the threshold-based policy class (\ref{eqn: policy_class_thre}) and the DQN-based method. 
    \item Occurrence-based mitigation policy $\pi^{M}_{m}$ for $m \in \{4, 6 \dots, 12\}$: a city implements action $2$ when there are new cases confirmed in the past $m$ days, and action $1$ otherwise.
    \item Occurrence-based suppression policy $\pi^{S}_{m}$ for $m \in \{4, 6, \dots, 10\}$: a city begins to implement action $2$ after $m$ days from its first confirmed case and strengthens it to level $3$ after $m$ more days. Afterwards, the city weakens the action to level $2$ when there have been no new cases for $m$ days and level $1$ there have been no new cases for $2m$ days.
    \item Count threshold-based policy $\pi^{TB}_{m}$ for $m \in \{5, 10, \dots, 50\}$: a city implements action $3$ when the count of new cases on the day before exceeds $m$, action $1$ when it is zero, and action $2$ otherwise.
    \item Behaviour policy $\pi^B$: the observed trajectories in the dataset.
\end{enumerate}
% The experiments are run on a c5d.24xlarge instance on the AWS EC2 platform, with 96 cores and 192GB RAM, and it takes roughly 12 hours to complete. 

For each policy except for $\pi^B$, we run $100$ replications and present the average costs in Figure \ref{figure:Pareto}. 
% The standard errors are small and reported in the supplement. 
% \hl{For $\pi^B$, the observed count of new confirmed cases from day $21$ to $120$ is used as the epidemiological cost, and the observed actions from day $12$ to $120$ are used to generate economic costs. }
% between the two objectives
We can see that the proposed method provides a clear view of the tradeoff and its performance is generally better than the competing  policies. 
In some cases, the DQN-based policies are slightly better than the threshold-based policies, while the overall value difference is not large. 
The behaviour policy by Chinese local governments is quite strict in the later period, and we interpret part of this effort as the attempt to curb the cross-border spread.
The other policies are not Pareto-optimal and also are not adaptive to  different situations in different cities. 
The clear trend among the occurrence-based suppression policies emphasizes the importance of intervening as promptly as possible, which can reduce both  costs. 
% More details about the evaluation procedure and additional analysis can be found in the supplement XXX. 

\setlength{\textfloatsep}{10.0pt plus 2.0pt minus 4.0pt}% Remove \textfloatsep

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-0.2cm}
\begin{figure}[h!]
\centering		
\includegraphics[width=.55\textwidth, height=.6\textwidth]{figures/main_with_DQN.png} 
% re_Figure3_factor10
\caption{Cumulative epidemiological costs and economic costs  following different policies, averaged over $100$ replications. The closer to the left bottom corner, the better. The standard errors are negligible. 
On each curve, the different markers represent the performance of a policy with different hyper-parameters. 
}
\label{figure:Pareto}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To further investigate the robustness of the proposed method, two sensitivity analyses are conducted. 
Specifically, we repeat the above experiment with either various combinations of hyper-parameters or with the data generation model modified as a generalized Susceptible-Exposed-Infected-Removal model  \citep{tang2020review}. 
The results can be found in Appendix \ref{sec: supp-robust}. %in the supplement. 
In reasonable ranges, the proposed method still yields consistent and superior performance. 
% The other findings are similar with above. 


Finally, recall that infectious disease control is about trade-off. 
For a disease as infectious as the COVID-19, usually a stricter policy would be preferred. 
However, for a less infectious one, the same response policy might result in over-reaction and hence unnecessary costs to the economics. 
To demonstrate the adaptiveness of the proposed method, we repeat the above experiment with a less infectious disease. 
Specifically, we calibrate the GSIR model with the parameters of the 2009 H1N1 pandemic, with the other settings kept the same for ease of comparison. 
We choose the parameters estimated in \cite{fraser2009pandemic}, which reports an $R_0$ of about $1.4$. 

The results are summarized in Figure  \ref{figure:Pareto_H1N1}. 
We can see that the proposed method still yields superior performance. 
The count threshold-based policies achieve close performance with some Pareto-optimal policies, while our method provides more options with a clear trade-off. 
Compared to Figure \ref{figure:Pareto}, the economic costs of the strict  suppression policy increase, relative to the other policies. 
% We interpret this as, for a less infectious disease, the decision-making would be subtler.
% , which demonstrates that such a strict  
% when compared with the other fixed baselines
% sub-optimal
% a fixed response policy 
% (i.e., avoiding over-reaction)? 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering		
\includegraphics[width=.55\textwidth, height=.6\textwidth]{figures/H1N1_with_DQN.png} 
% Pareto_H1N1
\caption{Experiment results with model parameters calibrated from the H1N1 pandemic. The costs of the behaviour policy are not displayed since they are not comparable.}
% with the H1N1 pandemic setting
\label{figure:Pareto_H1N1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> COVID_KDD (Camara Ready) [Arxiv]/5_data.tex <==
\vspace{-0.2cm}
\subsection{Data description and hyper-parameters}\label{sec:data}
% choose one day as the time unit and 
We collect data for six important cities in China from 01/15/2020 to 05/13/2020, 
and index these cities by $l \in \{1, \dots, 6\}$ and dates by $t \in \{1, \dots, 120\}$, with $T = 120$. 
% where the horizon $T$ as discussed in Sec \ref{sec:pre} is chosen as $120$.
More details about the dataset, data sources, and hyper-parameters can be found in Appendix \ref{sec:supp-data}. 
% in the supplement. 
% More details can be found in Section \ref{sec:supp-data} in the supplement. 
% , and the state variables are then constructed as in\textbf{} Section \ref{sec:delayed}. 

\vspace{-0.2cm}
\begin{description}
\item[State variables and region-specific features:] 
For each region $l$, 
we collect its annual gross domestic product (GDP) $G_l$,  population $M_l$, and counts of confirmed cases from official sources. 

\item[Action:] 
% \hl{mention in the intro to determine the scope and avoid questions on this.}
three levels of interventions implemented in China during COVID-19 are considered: 
level $1$ means no or few official policies claimed; 
level $2$ means the public health emergency response;  % , which implies canceling mass gatherings
level $3$ means the stringent closed-off management required by the government. 
Data are collected from the news. 
% since governments usually adopt strategic response with progressive strength of action levels, we collect action data from the news and define level $1$, level $2$, and level $3$ as few official policies claimed, official policies claimed without quarantine required, and official quarantine policy claimed respectively.


\item[Cost:]  we use $r_{l,t}$, the observed ratio of human mobility loss in city $l$ on day $t$ compared with year 2019, to construct a proxy for its GDP loss and calibrate the action cost function $c_l(\cdot)$. 
For $j \in \{2, 3\}$, we first fit a normal distribution $\mathcal{N}(\mu_j,\sigma_{j}^2)$ to the observed loss ratios under the corresponding intervention level. 
We then define $c_l(a) $ as $ \sum_{j=1}^3 C_j \mathbb{I}(a = j) G_l / 365$, where $C_1 {=} 0$ and $C_j {\sim} \mathcal{N}(\mu_j,\sigma_{j}^2)$ for $j \in \{2, 3\}$. 
We note that this is only for illustration purposes. In real applications, policymakers  need  to carefully design and measure the potential costs with domain experts. 
\item[Hyper-parameters:] 
the parameter estimates for a similar pandemic SARS  \cite{mkhatshwa2010modeling} are used as priors of $\gamma$ and $\beta_1$. 
Similar to \cite{ferguson2020impact}, we assume that action $2$ and $3$ can reduce the infection rate by $80\%$ and $90\%$, respectively, and set the priors for $\beta_2$ and $\beta_3$ accordingly. 
$D$ is chosen as $9$ according to \cite{sun2020tracking} and \cite{pellis2020challenges}. 
% All the above hyper-parameters are chosen according to domain knowledge. 
% Section \ref{sec:sensitivity} of 
\end{description}





% the impact of such measures is typically only seen nine days - i.e. three doubling times - after their implementation. 

% \textbf{State variables:} 
% the surveillance data $O_{l,t}^I$ is collected from \hl{[CITE]}, and the time-varying state variables are constructed from $O_{l,t}^I$ as  in Section \ref{sec:delayed}. 
% We consider one static feature $X_l$, the annual gross domestic product (GDP) of region $l$. Both $M_l$  and $X_l$ are collected from \cite{hongheiku}. \\
% \textbf{Action:} three levels of intervention measures implemented in China during COVID-19 are considered: 
% % action definitions; more introduction
% level $1$ means no or few official policies claimed; 
% level $2$ means public health emergency response, which implies canceling mass gatherings; 
% level $3$ means the closed-off management required by the government. 
% All action data is collected from news. 
% \item{Cost:}  we use $r_{l,t}$, the observed loss ratio of human mobility compared with the same date in year 2019, to construct a proxy for the  GDP loss. 
% The data is collected from the online platform Baidu Migration \cite{BaiduQianxi}.
% We first fit a normal distributions $\mathcal{N}(c_j,\sigma_{C,j}^2)$ to $\{r_{l,t}| A_{l,t} = j, 1\le l \le 6, 1 \le t \le 61\}$ for $j \in \{2, 3\}$.
% In our experiment, we define the cost variable $C^A_{l,t}$ = $\sum_{j=1}^3 C_j I_{\{A_{l, t} = j\}} X_l / 10$, where $C_1 = 1$ and $C_j \sim \mathcal{N}(c_j,\sigma_{C,j}^2)$ for $j \in \{2, 3\}$. 
% We emphasize that this is only for illustration purpose. In real applications, policymakers  need  to carefully design and measure the potential costs with domain experts. \\
% \item[Hyper-parameters:] The parameter estimates for SARS \cite{mkhatshwa2010modeling} are used as prior for $\gamma$ and $\beta_1$. 
% Similar with \cite{ferguson2020impact}, we choose 
% $u_2 = 0.2$ 
% and $ u_3 = 0.1$ as the subjective expected action effect to set the prior mean for $\beta_2$ and $\beta_3$, with the prior variance the same with that of $\beta_1$.  $D$ is chosen to be $9$ according to \cite{sun2020tracking} and \cite{pellis2020challenges}.
% The experiment results are not sensitive to these hyper-parameters within a range.
% \item[Cost:] Similar with \cite{alvarez2020simple},  the loss of GDP per day compared with last year is chosen as the action cost. 
% Specifically, we set $C^A_{l,t} \sim \mathcal{N}(X_l \mu_i / 365, \sigma_i^2)$ when $A_{l,t} = i$, for $i = 1, 2, 3$. We choose $\mu_1 = 0, \mu_2 = 0.4, \mu_3 = 0.6$, and $\sigma_i = 0.1$ for  $i = 1, 2, 3$. 


==> COVID_KDD (Camara Ready) [Arxiv]/5_exp_SIR.tex <==

% day 12 [2020-01-26]
% day 13 [2020-01-27]
% day 120 [2020-05-13]
\subsection{Estimation and validation of the transition model}\label{sec:numerical_SIR}
The performance of our learned policies and the choices of weights both rely on the prediction accuracy of the estimated GSIR model, and we aim to first examine this point via temporal validation. 
Specifically, we first estimate the GSIR model using all data until day $12$,
and then for each city $l$, we predict $X^R_{l,t}$, the count of cumulative confirmed cases, from day $13$ to $120$ following the observed actions in data via forward sampling with the estimated GSIR model. 
Such a prediction can partially reflect the quality of our decisions suppose when we are on day $12$. 
The results aggregated over $1000$ replications are plotted in Figure \ref{figure:final_pred} and the prediction bands successfully cover the observed counts in most cases. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]%\fontsize{9}{10}\selectfont
% \setstretch{1}
\centering
    \caption{Posterior means and standard deviations (in the parentheses) obtained using data for all the six cities until day $t_0$.}
    % \vspace{-.5cm}
    \label{table:1}
    \begin{tabular}{llllllll}
\toprule
  $t_0$ & $R_0^1$  &  $R_0^2$    & $R_0^3$  & 
  $\gamma$ &   $\beta_1$ &   $\beta_2$ &   $\beta_3$   \\
\midrule
12  & 4.13 (.34) & 0.74 (.09) & 0.37 (.06) & 0.07 (.005) & 0.29 (.011) & 0.05 (.005) & 0.03 (.004)  \\
61 & 2.32 (.09)  & 0.70 (.03) & 0.38 (.03) & 0.11 (.002) & 0.25 (.007) & 0.07 (.003) & 0.04 (.003) \\
\bottomrule
\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering
% \begin{minipage}{\textwidth}
% 	\centering		
% 	_12_12_FALSE_20_final_val
\includegraphics[width=.8\textwidth]{figures/re_Figure2_lower_with_A.png} 
	\caption{Validation results for the six important cities in China. The solid lines are the observed counts of the cumulative infected cases. 
	The red dotted lines represent the mean predicted numbers, with the shaded areas indicating the $99\%$ prediction bands. 
	When a different action was taken, we annotate the new action level on the change point.}
	\label{figure:final_pred}
% \end{minipage}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To provide more insights into the intervention effects, in Table \ref{table:1}, we present the estimated parameters  using all data until day $61$, since the new cases afterwards are sparse. 
Here, $R_0^j = \beta_j / \gamma$ is the basic reproduction number under action level $j$, which plays an essential role in epidemiology analysis \cite{delamater2019complexity}. 
Roughly speaking, $R^j_0 < 1$ implies the pandemic will gradually diminish under action $j$. 
% Based on Table \ref{table:1}, 
The small value of $R^3_0$ indicates that action $3$ has a significant effect on controlling the pandemic;
measure $2$ is also effective and is more like a mitigation strategy;
the value of $R^1_0$ emphasizes that a lack of intervention will lead to a disaster.  
The estimates of $R^1_0$ and intervention effects ($R^2_0 / R^1_0$ and $R^3_0 / R^1_0$) are consistent with the existing results surveyed in \cite{alimohamadi2020estimate} and \cite{cheatley2020effectiveness}. 
We also reported the estimates used to make the predictions in Figure \ref{figure:final_pred}. 
Although the estimation is not perfect due to data scarcity in the early stage, 
the prediction still captures the rough trend under a reasonable policy and we expect it will not affect the decision-making significantly. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $R_0$ can be understood as the expected number of cases directly generated by one infectious individual before he is removed. 
% Therefore, 
% The absolute deviation between the predicted expectation of the infected counts until day $120$ and the observed one is 75.744 days \hl{Verified}, averaged over the 6 cities. 

% As Figure \ref{figure:final_pred} shows, the models were trained using data from all nine cities ranging from Jan 12th to Jan 29th and estimate the counts of total confirmed cases as well as daily new cases from Jan 30th to Mar 16th.


% Another way to appreciate our model as well as understand the behaviour of a policy is to look at the predicted bands following a fixed policy. 
% This is also what will be presented to decision makers by Algorithm \ref{alg:tool}. 
% interpretation of R0. falls into the range surveyed by 



==> COVID_KDD (Camara Ready) [Arxiv]/6_Conclusion.tex <==
\section{Discussion}\label{sec:discussion}
Motivated by the ongoing COVID-19 pandemic and the witnessed challenges in decision-making for policymakers, 
this paper proposes a novel model-based multi-objective RL framework to assist policymakers in real-time decision-making with the objective of minimizing the overall long-term cost. 
The method shows promising performance in numerical studies. 

% We admit this is a prototype
The overall framework is generally applicable to infectious disease pandemics. 
There are several components that can be extended: 
(i) other epidemiology models than the SIR model can also be used as the transition model, with the estimation method and policy class modified correspondingly;
(ii) more than two objectives can be similarly formalized, and resource limits can also be considered by introducing a cost to penalize exceeding the limits; 
% by including constraints in the specification of the policy class;
(iii) other parametric policy classes can be similarly formalized depending on the information required for decision-making. 

We note that modeling the economic costs caused by various intervention measures is, admittedly, a challenging but important task. 
This is out of the scope of this paper and we use a simple proxy in the experiment for illustration purposes. 
A systematic analysis of the observed costs during COVID-19 would be a meaningful next step. 
Besides, choosing among the Pareto-optimal policies is another challenging task, which is arguably beyond the scope of data-driven methods. 
Options can be presented to a committee or the citizens for discussion or voting. 
% 1. Choosing among Pareto-optimal policies: This issue is out of the scope of data-driven methods and is up to the choice of policymakers. Options can be presented to a committee or the citizens for discussion/voting. 

As future directions, 
the spreads among multiple regions can be incorporated under the multi-agent RL framework, 
% the partially observable MDPs can be considered to deal with the delayed observation problem, 
the heterogeneity of different regions can be accounted in a similar way as in \cite{qian2020lift} if we have enough data, 
and a multidimensional action space with the combinations of different interventions can be considered. 
% is a meaningful next step


% Finally, we note that additional resource constraints can also be taken into consideration through the cost function. 
% For example, with the limited number of I.C.U. beds, by introducing a separate model for the severe cases and the recovery rate, and modifying the epidemiological cost to penalize exceeding the limit, we can achieve this goal. 
% The aforementioned framework and algorithms can be easily extended to this setting. 


Finally, we would like to emphasize that taking the economy as more  important than human lives is not a motivation or an outcome of this framework. 
On one hand, economic losses can also cause health damage to many people, probably no less than the direct damage from the disease; 
on the other hand, the estimated Pareto-optimal policies aim to help policymakers reduce the cost on one objective without sacrificing the other, as illustrated in Section \ref{sec:numerical_policy}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% More discussion on why this is general. it would be good if the authors could summarise the degrees of freedom of the framework in the discussion, to enable a better judgement of its impact outside of the proposed application.

% underlying assumptions, moving parts, 

% action delay, cost switch

% Considering the tremendous impact that the COVID-19 crisis is having on human society, and the continuous testing of the trust that the public puts in the wide scientific community, it is extremely important that work on COVID-19 goes well above expectations to document and justify methodological *tradeoffs, failure cases, overall impact, and provide a reasonable view* on *how the work should be interpreted by people outside of the tight ML community.* In this particular case, I wish the author -- for instance -- had done a thorough investigation of *consequences of using their model wrt. the interpretability of the choices it makes*

==> COVID_KDD (Camara Ready) [Arxiv]/Algorithms/Algo_MBS.tex <==
% \vspace{.2cm}
% \rho_{t_0}(\vthe)
 \begin{algorithm}[ht]
% \SetAlgoLined
%  $\hat{\vthe}_{t_0}$
\KwData{$\{ O^I_{l,t}\}_{t = t_0 - D}^{t_0}$, $\{A_{l,t}\}_{t = t_0 - D}^{t_0 - 1}$, $\rho_{t_0}$,  and $D$
}
set $X^{I,G}_{l,t_0 - D} = O^{I}_{l,t_0} - O^{I}_{l,t_0 - D}$ and $(\hat{\gamma}_{t_0}, \hat{\beta}_{1,t_0}, \dots, \hat{\beta}_{J,t_0})^T = \mathbb{E}(\rho_{t_0})$.

\For{$t= t_0-D, \dots, t_0 - 1$}{
  $X^{I,G}_{l,t+1} = X^{I,G}_{l,t} + \sum_{j=1}^J \hat{\beta}_{j, t_0}  \mathbb{I}_{\{A_{l,t} = j\}} (M_l - O^I_{l,t} - X^{I,G}_{l,t}) X^{I,G}_{l,t} / M_l
- (O^I_{l,t + 1} - O^I_{l,t})$
% j?
}
% (\sum_i\hat{\beta}_{i,t_0}I_{\{A_{l,t}=i\}})


% set $X^{I}_{l,t_0} = X^{I,G}_{l,t_0}, X^S_{l, t_0} = M_{l} - X^{I}_{l,t_0} - X^{R}_{l,t_0}$

% \KwResult{$S_{l,t_0} = (X^{S}_{l,t_0}, X^{I}_{l,t_0}, X^{R}_{l,t_0})$}  

\KwResult{the proxy state $S_{l,t_0} = (M_{l} - X^{I, G}_{l,t_0} - O^I_{l,t_0}, X^{I,G}_{l,t_0}, O^I_{l,t_0})^T$}
\caption{Model-based Simulation (MBS)}\label{alg:MBS}
\end{algorithm}
% \vspace{.5cm}

==> COVID_KDD (Camara Ready) [Arxiv]/Algorithms/Algo_Pareto.tex <==

\begin{algorithm}[ht]
\DontPrintSemicolon
\KwIn{weights $\{\omega_b\}_{b=1}^B$, number of replications $K$, significance level $\alpha$, action cost function $c_l(\cdot)$, decision points $\mathcal{T}$, $\mathcal{D}_{t_0}, \rho_{t_0}, T$.
}
% , $\hat{\vthe}_{t_0}, S_{l,t_0}, w_{l,t_0}$, tol $>0$, $\vlam^1 \in E_1$,  $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}, t_0, \mathbb{G}$}
% \hl{data etc; policy search algorithm and $\mathcal{F}$}

\For{$b = 1, \dots, B$}{
apply a policy search algorithm to find the optimal policy  $\hat{\pi}^b$ for weight $\omega_b$. 
% the policy search algorithm
% (e.g., Algorithm \ref{alg:grid})
% \KwData{$X^I_{l, {t_0 - D}}$, $\{ X^R_{l,t}\}_{t = t_0 - D}^{t_0}$, $\{A_{l,t}\}_{t = t_0 - D}^{t_0 - 1}$, $\rho_{t_0}$, $X_{l}$, and $D$
% }


 \For{$k = 1, \dots, K$}{
 set the cumulative cost $V^{k, E}_{t_0 - 1}$ and  $V^{k, A}_{t_0 - 1}$ as $0$
 
%  apply Algorithm \ref{alg:MBS} to generate the belief state $S^{k}_{t_0}$
 set $S^{k}_{t_0,b} = S_{t_0}$
 
  \For{$t= t_0,\dots,T$}{

            % apply Algorithm \ref{alg:MBS} to generate the belief state $S^{m,G}_{t}$
            
            choose action $A^k_{t,b} = \hat{\pi}^b(S^{k}_{t,b}) \mathbb{I}(t \in \mathcal{T}) + A^k_{t-1,b} \mathbb{I}(t \notin \mathcal{T})
            $
            % \pi(S^m_{t}; \vlam_{t_0}^b)$, 
            
            sample $C^{k, A}_{t,b} \sim c_l(A^k_{t,b})$, 
            $\vthe^k_{t,b} \sim \rho_{t_0}$, and $S^k_{t+1,b} \sim  f(\cdot|S^k_{t,b}, A^k_{t,b}; \vthe^k_{t,b})$
             
            calculate $V^{k, E}_{t,b} = V^{k, E}_{t - 1,b} + X^{k, S}_{t,b} - X^{k, S}_{t + 1,b}$ and $V^{k, A}_{t,b} = V^{k, A}_{t - 1,b} + C^{k, A}_{t,b}$
        }
    }
    for every $t$, calculate the upper and lower 
    $\alpha/2$-th quantile and the mean of $\{V^{k, E}_{t,b}\}_{k=1}^K$ as $V^{b,E}_{u,t}$, $V^{b,E}_{l,t}$, and $\bar{V}^{b,E}_{t}$, respectively; 
    similarly calculate $V^{b,A}_{u,t}$,  $V^{b,A}_{l,t}$, and  $\bar{V}^{b,A}_{t}$.
}

\KwResult{ optimal policies $\{\hat{\pi}^b\}_{b = 1}^B$
, recommended actions $\{A^1_{t_0,b}\}_{b = 1}^B$, 
prediction bands for  costs
$\{\{(V^{b,E}_{l,t}, V^{b,E}_{u,t}, \bar{V}^{b,E}_{t}),
(V^{b,A}_{l,t}, V^{b,A}_{u,t}, \bar{V}^{b,A}_{t}) \}_{t = t_0}^T
\}_{b = 1}^B$ }  
\caption{Pareto-optimal Policies and Prediction Bands
% : For region $l$
}\label{alg:tool}
\end{algorithm}


% epidemiological and economic



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \vspace{.2cm}
%  \begin{algorithm}%[H]
% % \SetAlgoLined
% \DontPrintSemicolon
% \KwData{weights $\{\omega_b\}_{b=1}^B$, significance level $\alpha$, all parameters for %Algorithm \ref{alg:SPSA}
% the policy search algorithm. 
% }
% % , $\hat{\vthe}_{t_0}, S_{l,t_0}, w_{l,t_0}$, tol $>0$, $\vlam^1 \in E_1$,  $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}, t_0, T, M, \mathbb{G}$}

% \For{$b = 1, \dots, B$}{
% apply Algorithm \ref{alg:grid} or Algorithm \ref{sec:SPSA}.\ref{alg:SPSA} to find the optimal policy  $\hat{\pi}^b$ for weight $\omega_b$. 
% % the policy search algorithm

% % \KwData{$X^I_{l, {t_0 - D}}$, $\{ X^R_{l,t}\}_{t = t_0 - D}^{t_0}$, $\{A_{l,t}\}_{t = t_0 - D}^{t_0 - 1}$, $\rho_{t_0}$, $X_{l}$, and $D$
% % }


%  \For{$m=1,\dots,M$}{
%  set $V^{m,E}_{t_0 - 1} = 0$ and $V^{m,A}_{t_0 - 1} = 0$.
 
%   \For{$t= t_0,\dots,T$}{

            
%             apply Algorithm \ref{alg:MBS} to generate the belief state $S^{m,G}_{t}$
            
%             choose action $A^m_{t,b} = \hat{\pi}^b(S^{m,G}_{t}) \mathbb{I}(t \in \mathcal{T}) + A^m_{t-1,b} \mathbb{I}(t \not\in \mathcal{T})
%             $
%             % \pi(S^m_{t}; \vlam_{t_0}^b)$, 
            
%             sample $\vthe \sim \rho_{t_0}$, $S^m_{t+1} \sim  f(\cdot|S^m_{t}, 
%             A^m_{t,b}; \vthe)$, and 
%             $C^{m,A}_{t} \sim c(A^m_{t,b}, X_l)$ 

            
            
%             calculate $V^{m,E}_{t} = V^{m,E}_{t - 1} + X^{m, S}_{t - 1} - X^{m, S}_{t}$ and $V^{m,A}_{t} = V^{m,A}_{t - 1} + C^{m,A}_{t}$
%         }
%     }
%     for  $t \in \{t_0, \dots, T\}$, calculate the upper and lower 
%     $\frac{\alpha}{2}$-th quantile and the mean of $\{V^{m,E}_{t}\}_{m=1}^M$ as $V^{b,E}_{u,t}$, $V^{b,E}_{l,t}$, and $\bar{V}^{b,E}_{t}$; 
%     similarly calculate $V^{b,A}_{u,t}$,  $V^{b,A}_{l,t}$, and  $\bar{V}^{b,A}_{t}$.
% }

% \KwResult{$\{ \hat{\pi}^b, A^1_{t_0,b}, 
% \{(V^{b,E}_{l,t}, V^{b,E}_{u,t}, \bar{V}^{b,E}_{t}), 
% (V^{b,A}_{l,t}, V^{b,A}_{u,t}, \bar{V}^{b,A}_{t}) \}_{t = t_0}^T
% \}_{b = 1}^B $}  
% \caption{Pareto Efficient Policies}\label{alg:tool}
% \end{algorithm}
% % \vspace{.5cm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% calculate $\bar{V}^{b,E} = \sum_{t=t_0}^{T} \bar{V}^{b,E}_{t} / (T-t_0+1)$
%  and 
%  $\bar{V}^{b,A} = \sum_{t=t_0}^{T} \bar{V}^{b,A}_{t} / (T-t_0+1)$
%  (\bar{V}^{b,E}, \bar{V}^{b,A}),

==> COVID_KDD (Camara Ready) [Arxiv]/Algorithms/Algo_SPSA.tex <==

\vspace{.2cm}
 \begin{algorithm}[!h]
% \SetAlgoLined
\KwData{tolerance $tol >0$, initial point $\vlam^1 \in E_1$,  step sizes $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}$, 
number of replications $M$,  direction distribution $\mathbb{G}$; 
other parameters $t_0, T, \mathcal{T}, c_l(\cdot)$,  
$\rho_{t_0}, X^I_{l, {t_0 - D}}, \{ X^R_{l,t}\}_{t = t_0 - D}^{t_0}, \{A_{l,t}\}_{t = t_0 - D}^{t_0 - 1}, w_{l,t_0}$ }

\textbf{Initialization:}
set $\delta = \infty$, $k = 1$, 
$X^{I,+}_{l, {t_0 - D}} = X^{I,-}_{l, {t_0 - D}} = X^I_{l, {t_0 - D}}$, $X^{R,+}_{l,t} = X^{R,-}_{l,t} = X^R_{l,t}$ for $ t \in \{t_0 - D, \dots, t_0\}$, 
and $A^{+}_{l,t} = A^{-}_{l,t} = A_{l,t}$ for $ t \in \{t_0 - D, \dots, t_0 -1\}$

\While{$\delta \ge tol$}{
    sample $\Delta_k \sim \mathbb{G}$; 
    set $\vlam^{k,+} = \vlam^k + \xi_k \Delta_k$ % more general?
    and $\vlam^{k,-} = \vlam^k - \xi_k \Delta_k$
    
    set $V_k^+ = V_k^- = 0$
    
    \For{$m=1,\dots,M$}{
        
        
        \For{$t'=t_0,\dots,T$}{
        sample $\vthe_{m, t'} \sim \rho_{t_0}$
        
            generate $S^{b,+}_{l, t'} =  MBS(\{ X^{R,+}_{l,t}\}_{t = t' - D}^{t'}$, 
              $\{A^{+}_{l,t}\}_{t = t' - D}^{t' - 1}, \rho_{t_0}, D)$

            choose action $A^+_{l,t'} = \pi(S^{b,+}_{l, t'}; \vlam_t^{k,+}) \mathbb{I}(t \in \mathcal{T}) + A^+_{l, t' - 1} \mathbb{I}(t \notin \mathcal{T})$
            
            sample $S^+_{l,t'+1} \sim  f(\cdot|S^+_{l,t'}, 
            A^+_{l,t'}; \vthe_{m, t'} )$ 
            and 
            $C^{A,+}_{l,{t'}} \sim c_l(A^+_{l,t'})$ 
            
            calculate  $Y^+_{l,{t'}} = 
            X^{S,+}_{l,t'} - X^{S,+}_{l,t'+1} + 
            \omega_{l,t_0} C^{A,+}_{l,{t'}}$

            generate $S^{b, -}_{l, t'} =  MBS(\{ X^{R,-}_{l,t}\}_{t = t' - D}^{t'}$, 
              $\{A^{-}_{l,t}\}_{t = t' - D}^{t' - 1}, \rho_{t_0}, D)$
              
            choose action $A^-_{l,t'} = \pi(S^{b, -}_{l, t'}; \vlam_{t_0}^{k,-}) \mathbb{I}(t \in \mathcal{T}) + A^-_{l, t' - 1} \mathbb{I}(t \notin \mathcal{T}) $
            
            sample $S^-_{l,t'+1} \sim  f(\cdot|S^-_{l,t'}, 
            A^-_{l,t'}; \vthe_{m, t'} )$ 
            and 
            $C^{A,-}_{l,{t'}} \sim c_l(A^-_{l,t'})$ 
            
            calculate  $Y^-_{l,{t'}} = 
            X^{S,-}_{l,t'} - X^{S,-}_{l,t'+1} + 
            \omega_{l,t_0} C^{A,-}_{l,{t'}}$
            

        }
        update $V_k^+ = V_k^+ + (T-t_0+1)^{-1}\sum_{t' = t_0}^{T} Y^+_{l,t'}$, 
        $V_k^- = V_k^- + (T-t_0+1)^{-1}\sum_{t' = t_0}^{T} Y^-_{l,t'}$
    }
    
    calculate $\bar{V}_k^+ = V_k^+ / M $, 
        $\bar{V}_k^- = V_k^- / M $
    
    Set $\vlam^{k+1} = \mathbb{P}_{E_k}(\vlam^{k} + \zeta_k (2\xi_k)^{-1} (\bar{V}_k^+ - \bar{V}_k^-) \Delta_k )$ 
    
    set $ k = k + 1$ and $\delta = ||\vlam^k - \vlam^{k-1}||/||\vlam^{k-1}||$ 
 }
 \KwResult{optimal policy parameters ${\boldsymbol{\lambda}}_{l,{t_0}} = {\boldsymbol{\lambda}}^k$ }  
 \caption{Simultaneous Perturbation Stochastic Approximation}\label{alg:SPSA}
\end{algorithm}
\vspace{.5cm}

%  and  recommended immediate action $\pi(S_{l,t_0}|\vlam_{l,{t_0}})$.

==> COVID_KDD (Camara Ready) [Arxiv]/Algorithms/Algo_grid.tex <==
 \begin{algorithm}[!h]
% \SetAlgoLined
% lower and upper 
\KwIn{bounds of the search space $u_2, u_3, U_2,  U_3$; step sizes $\xi_2, \xi_3$; number of replications $M$; 
data $\{ O^I_{l,t}\}_{t = t_0 - D}^{t_0}$ and $ \{A_{l,t}\}_{t = t_0 - D}^{t_0 - 1}$; 
other parameters $D, \rho_{t_0}, w_{l,t_0}, t_0, T, \mathcal{T}, c_l(\cdot)$}


% set $X^{I,G}_{l,t_0 - D} = O^{I}_{l,t_0} - O^{I}_{l,t_0 - D}$

%  X^I_{l, {t_0 - D}},

set $\lam_2 = u_2$,  $V^* = +\infty$, $S_{l, t_0} =  MBS(\{ X^R_{l,t}\}_{t = t_0 - D}^{t_0}$, 
              $\{A_{l,t}\}_{t = t_0 - D}^{t_0 - 1}, \rho_{t_0}, D)$, and $X^R_{l,t} = O^I_{l,t}$ for $t \in \{t_0 - D, \dots, t_0\}$


\While{$\lam_2 \le U_2 $}{
    set  $\lam_3 = max(\lam_2, u_3)$
    
    \While{$\lam_3 \le U_3 $}{
        set $\vlam = (\lam_2, \lam_3)^T$ and the overall value $V = 0$
        
        \For{$m=1,\dots,M$}{
              
            \For{$t'=t_0, \dots,T$}{
              generate $S^G_{l, t'} =  MBS(
              \{ X^R_{l,t}\}_{t = t' - D}^{t'},$
              $\{A_{l,t}\}_{t = t' - D}^{t' - 1}, \rho_{t_0}, D)$

              choose action $A_{l,t'} {=} \pi(S^G_{l, t'}; \vlam) \mathbb{I}(t' {\in} \mathcal{T})
              + A_{l,t'-1} \mathbb{I}(t' {\notin} \mathcal{T})$

                sample $\vthe \sim \rho_{t_0}$,  $C^A_{l,{t'}} \sim c_l(A_{l,t'})$ 
                , and $S_{l,t'+1} \sim  f(\cdot|S_{l,t'}, 
                A_{l,t'}; \vthe)$
                
            %from $g$
            
               calculate  $V = V + (X^S_{l,t'} - X^S_{l,t'+1} + \omega_{l,t_0} C^A_{l,{t'}})$  
             }  
        
        }
        \textbf{if} $V < V^*$ \textbf{then} update $V^* = V$ and $\vlam^* = \vlam$
        % \If{}{
        
        % }

        set $\lam_3 = \lam_3 + \xi_3$
    }
    
    set $\lam_2 = \lam_2 + \xi_2$
}
% 
 \KwOut{ optimal policy $\hat{\pi}_{l, t_0}(\cdot; \omega_{l, t_0}) = \pi(\cdot; \vlam^*)$}
%  and the recommended  action $\hat{\pi}_{l, t_0}(X^{I,b}_{l,t_0})$}
 \caption{Policy Search with Grid Search }\label{alg:grid} % for the Optimal Policy
\end{algorithm}

==> COVID_KDD (Camara Ready) [Arxiv]/Algorithms/DQN.tex <==

\vspace{.2cm}
 \begin{algorithm}[!ht]
% \SetAlgoLined
\KwData{
weight $\omega$, posterior $\rho_{t_0}$, current state $s_0$, current decision point $t_0$, horizon $T$
number of episodes $M$, exploration probability $\epsilon$
}

\textbf{Initialization:}
set the replay buffer $\mathcal{D}$ as empty, the action-value function $Q(\cdot, \cdot)$ with random weights

\For{episode $e = 1, \dots, M$}{
    randomly initialize with an appropriate state $s$
    
    \For{$t = t_0, \dots, T$}{
        with probability $\epsilon / ((e + 1) // 10 + 1)$ select a random action a; otherwise select $a = \argmin_a Q((s, t), a)$
        
        take action $a$, sample $\theta \sim \rho_{t_0}$, and then sample the next state $s'$ according to the GSIR model with parameter $\theta$
        
        sample the action cost for $a$ and calculate the weighted cost for weight $\omega$ as $c$
        
        store transition $(s, a, c, s', t)$ in $\mathcal{D}$
        
        sample a mini-batch $\{(s_i, a_i, c_i, s'_i, t_i)\}$ from $\mathcal{D}$
        
        set $y_i = c_i + min_a Q((s'_i, t_i + 1), a)$ if $s'_i$ is not terminal, and set $y_i = c_i$ otherwise
        
        perform a gradient descent step on  $\{((s_i, t_i), y_i)\}$
        
        set $s' = s$
    }
}

 \KwResult{
 optimal policy $\hat{\pi}_{t_0}(\cdot; \omega) = argmin_a Q((\cdot,t_0), a; \omega)$ and the recommended action 
 $\hat{\pi}_{t_0}(s_0; \omega)$
 }  
 \caption{Modified deep-Q learning with experience replay and epsilon-greedy exploration for finite-horizon planning.}\label{alg:DQN}
\end{algorithm}
\vspace{.5cm}

%  and  recommended immediate action $\pi(S_{l,t_0}|\vlam_{l,{t_0}})$.

==> COVID_KDD (Camara Ready) [Arxiv]/Archive/0_KDD_pre_Archive.tex <==


\section{Citations and Bibliographies}

The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

The bibliography is included in your source document with these two
commands, placed just before the \verb|\end{document}| command:
\begin{verbatim}
  \bibliographystyle{ACM-Reference-Format}
  \bibliography{bibfile}
\end{verbatim}
where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
suffix, of the \BibTeX\ file.

Citations and references are numbered by default. A small number of
ACM publications have citations and references formatted in the
``author year'' style; for these exceptions, please include this
command in the {\bfseries preamble} (before the command
``\verb|\begin{document}|'') of your \LaTeX\ source:
\begin{verbatim}
  \citestyle{acmauthoryear}
\end{verbatim}

  Some examples.  A paginated journal article \cite{Abril07}, an
  enumerated journal article \cite{Cohen07}, a reference to an entire
  issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
  monograph/whole book in a series (see 2a in spec. document)
  \cite{Harel79}, a divisible-book such as an anthology or compilation
  \cite{Editor00} followed by the same example, however we only output
  the series if the volume number is given \cite{Editor00a} (so
  Editor00a's series should NOT be present since it has no vol. no.),
  a chapter in a divisible book \cite{Spector90}, a chapter in a
  divisible book in a series \cite{Douglass98}, a multi-volume work as
  book \cite{Knuth97}, a couple of articles in a proceedings (of a
  conference, symposium, workshop for example) (paginated proceedings
  article) \cite{Andler79, Hagerup1993}, a proceedings article with
  all possible elements \cite{Smith10}, an example of an enumerated
  proceedings article \cite{VanGundy07}, an informally published work
  \cite{Harel78}, a couple of preprints \cite{Bornmann2019,
    AnzarootPBM14}, a doctoral dissertation \cite{Clarkson85}, a
  master's thesis: \cite{anisi03}, an online document / world wide web
  resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game
  (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05}
  and (Case 3) a patent \cite{JoeScientist001}, work accepted for
  publication \cite{rous08}, 'YYYYb'-test for prolific author
  \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
  contain 'duplicate' DOI and URLs (some SIAM articles)
  \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
  multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
  couple of citations with DOIs:
  \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
  citations: \cite{TUGInstmem, Thornburg01, CTANacmart}. Artifacts:
  \cite{R} and \cite{UMassCitations}.

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section{Appendices}


==> COVID_KDD (Camara Ready) [Arxiv]/Archive/5_Broader_impact.tex <==
\section*{Ethics Statement}
We would like to emphasize that taking the economy as more  important than human lives is not a motivation or an outcome of this framework. 
On one hand, economic losses can also cause health damage to many people, probably not less than the direct damage from the disease; 
on the other hand, the estimated Pareto-optimal policies aim to help policymakers reduce the cost on one objective without sacrificing the other, as illustrated in Section \ref{sec:numerical_policy}. 

The framework is designed with the overall welfare of all people in mind. 
We acknowledge that the degree of interest loss for different groups may vary due to different choices among the Pareto-optimal policies, 
which is a tricky and unavoidable ethical question. 
For this purpose, 
an online interactive tool and an open-sourced software are under development to facilitate the real-time dissemination of results. 
Everybody is welcome to utilize these tools to have a better understanding of the current situation and participates in the discussion. 


% Two pages for references; optional ethics statement on these pages.
% Additionally, this year, we encourage authors to (optionally) write a statement about the potential ethical impact of their work, including its broad societal implications, both positive and negative.
% reviewers identify negative ethical concerns about a paper and it did not adequately address these concerns either in an ethics statement or in its main body.

% A widespread ethical concern during the outbreak of COVID-19 is .  


% \begin{figure}[t!]
% \centering		
% \includegraphics[width=.45\textwidth]{figures/action_plot.png} 	
% \caption{\hl{Move to supplement later. Not easy to read?}}
% \label{figure:action_plot}
% \end{figure}


% The validity of the proposed system depends on the prediction accuracy of the GSIR model as well as the modeling of the intervention costs. 
% A considerable error in either part may lead to a sub-optimal policy. 
% Fortunately, the online planning nature of the framework can mediate this issue, because the policymakers only need to select among a small set of actions every several days, and as long as the relative relationship between the prediction trajectories is reasonable, the system can recommend an appropriate action. 


% Nevertheless, it is the right action instead of accurate prediction itself that really matters. 


% Our method is generally applicable to infectious disease pandemics. 
% The direct users of this system is policymakers in each region, while everybody is 

% underreaction and overreaction, both having been witnessed. 
% too calm and objective


%%%%%%%%%%%%%%%%%%%%%%%% ARCHIVE %%%%%%%%%%%%%%%%%%%%%%%%
% Ethical Considerations in the example 
% Any text generation application that learns from data runs the risk of producing biased or offensive content reflective of the training data
% our work, which learns a language model from song lyrics, is no exception. 
% One approach that we implement is to moderate the words shown to our language model based on a list of keywords3; 
% a downside of this moderation is the potential for increased bias as a side effect of the content filter. 
% Recent work in modeling the intentions of vulgar expressions has shown promise for more nuanced profanity filtering or hate speech detection [12], and as these approaches improve, they present one path toward better automated moderation when working on text generation. 

% In addition to biased or offensive content, the other common ethical concern when working with material like lyrics is the potential for plagiarism. 
% In our setting, one of the reasons we choose to work with arbitrary audio inputs is to explicitly condition the language model with a strong signal which, intuitively, should make it difficult to copy from the training set; still, more work is needed to determine the extent to which the audio conditioning reduces plagiarism.

% For policymakers, however, it is the selection of the optimal control intervention in the face of uncertainty, rather than accuracy of model predictions, that is the measure of success that counts. 
% it is the selection of the optimal control interventions in the face of uncertainty that counts, and ultimately what they are judged on.


% Requirement: ethical aspects  and future societal consequences. (both positive and negative outcomes)
% \begin{enumerate}
%     \item who may benefit from this research and who may be put at disadvantage from this research
%     \item what are the consequences of failure of the system
%     \item whether the task/method leverages biases in the data
% \end{enumerate}


==> COVID_KDD (Camara Ready) [Arxiv]/Archive/new_commands.tex <==
%%%%%%%%%%%%
\newcommand{\Mean}{{\mathbb{E}}}
\newcommand{\Var}{{\mathbb{VAR}}}
\newcommand{\Cov}{{\mathbb{COV}}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\lam}{\lambda}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
\newcommand{\vlam}{\boldsymbol{\lam}}
\newcommand{\vrho}{\boldsymbol{\rho}}
\newcommand{\hRI}{\widehat{RI}}
\newcommand{\vthe}{\boldsymbol{\theta}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mI}{\mathbb{I}}
\newcommand{\mA}{\mathcal{A}}
\renewcommand{\prob}{{\mathbb{P}}}
\newcommand{\mT}{\mathcal{T}}
\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\argmax}{arg\!max}
\renewcommand\not[1]{#1\xnot}

%%%%%%%%%%%%


==> COVID_KDD (Camara Ready) [Arxiv]/Archive/packages.tex <==
\usepackage[ruled, vlined]{algorithm2e}
\setlength{\algomargin}{0em}

\usepackage{array}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{booktabs}

\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{soul}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{mathtools}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \userpackage{pdfpages}
% \usepackage{lineno}
% \usepackage{setspace}

% \usepackage[utf8]{inputenc}
% \usepackage[left=1.02in, right=1.02in, top=1.1in, bottom=1.05in]{geometry}
% \usepackage[font=small,labelfont=bf]{caption}
% \doublespacing
% \linenumbers


==> COVID_KDD (Camara Ready) [Arxiv]/Archive/suppCOVID.tex <==
% \usepackage{amssymb}
\input{0_KDD_pre}
\usepackage{subcaption}

\usepackage{xr}
\makeatletter

\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\myexternaldocument{./0_MAIN}



\title{Supplement to ``Multi-Objective Model-based Reinforcement Learning for Infectious Disease Control"}

\begin{document}
\setcounter{section}{1}
	
\maketitle

\appendix 



\raggedbottom
\section{Posterior estimation of the GSIR model}\label{sec:MAP}
In this section, we introduce the derivation of the posteriors. 
% our prior family choices for $\vthe$ and
Recall our model (\ref{SIR}) is 
\begin{align*}
% \begin{split}
X^S_{l,t+1} &= X^S_{l,t} - e^S_{l,t}, e^S_{l,t} \sim  \text{Poisson}(\sum_{j=1}^J \beta_j \mathbb{I}(A_{l,t} = j) X^S_{l,t} \frac{X^I_{l,t}}{M_l}) ;\\ %   \hl{notation?}
X^R_{l,t+1 } &= X^R_{l,t} + e^R_{l,t}, e^R_{l,t} \sim \text{Binomial}(X^I_{l,t}, \gamma );\\
X^I_{l,t+1} &= M_l - X^S_{l,t+1} - X^R_{l,t+1 }, 
% \end{split}
\end{align*}
where the third equation is redundant. 
With data $\mathcal{D}_{t_0}$, the Markov property of the transition model reduces the estimation problem to $J + 1$ Bayesian generalized linear models with the identity link function. 
Specifically, let ${\Omega_{t_0,j}} = 
\{(t,l): 1 \leq t \leq t_0 - 1,
1 \leq l \leq N_{t}, 
A_{l,t} = j\}$ be the set of time-location pairs where action $j$ is taken, and let $\Omega_{t_0} = \{(t,l): 1 \leq t \leq t_0 - 1,
1 \leq l \leq N_{t}\}$. 
Assume $\{e^S_{l.t}, e^R_{l.t}|  1 \leq t \leq t_0 - 1,
1 \leq l \leq N_{t} \}$ are all independent, and then the likelihood function can be written as 
\begin{align*}
&\mathcal{L}( \vthe |\mathcal{D}_{t_0}) 
= \prod_{(t,l) \in \Omega_{t_0}} f_B(X^R_{l,t+1 } - X^R_{l,t}, X^I_{l,t}; \gamma)  \\
&\quad \times \prod_{j \in \{1, \dots, J\} } \prod_{(t,l) \in \Omega_{t_0,j}} f_P(
X^S_{l,t} - X^S_{l,t+1}; %\\ 
\sum_{j=1}^J \beta_j \mathbb{I}(A_{l,t} = j)  X^S_{l,t} X^I_{l,t} / M_l ), 
\end{align*} 
where $f_B(\cdot, \cdot; \cdot)$  is the density function of the Binomial distribution and $f_P(\cdot; \cdot)$ is that of the Poisson distribution. 
For simplicity, we consider the case that the parameter priors are independent with each other. 
For more general settings, approximate inference methods such as Markov Chain Monte Carlo can be used. 
For the recover rate $\gamma$, we use the Beta-Binomial conjugate pair and set its prior as $Beta(a_{R}, b_{R})$ with parameters 
$a_{R}$ and  $b_{R}$. 
For the infection rate $\beta_j$, $j = 1, \dots, J$, the Poisson-Gamma conjugate pair is used,
and we set the prior of $\beta_j$ as $ Beta(a_{S,j}, b_{S,j})$ with parameters 
$a_{S, j}$ and  $b_{S, j}$. 
By choosing these conjugate priors, the corresponding posterior distributions have explicit forms as $\gamma \mid \mathcal{D}_{t_0} \sim  Beta(a_{R}^* , b_{R}^*)$ 
and 
$\beta_j \mid \mathcal{D}_{t_0} \sim  Gamma(a_{S,j}^* , b_{S,j}^*)$, for $j = 1, \dots, J$
, where

\begin{equation*}
    \begin{aligned}
a_{S,j}^* &= a_{S,j} + \sum_{(t,l) \in \Omega_{t_0,j}}\left( {X_{l, t}^{S} - X_{l, t+1}^{S}}{} \right),\\
b_{S,j}^* &= b_{S,j}+ \sum_{(t,l) \in \Omega_{t_0,j}}  \frac{X_{l, t}^{S,j}X_{l, t+1}^{I}}{M_l}, \\
a_{R}^* &= a_{R} + \sum_{(t,l) \in \Omega_{t_0}} \left( {X_{l, t+1}^{R} - X_{l, t}^{R}} \right), \\ % (t,l)  because l \leq N_t depends on t --> t first then l or (l, t) location \sum_{l=1}^{N_{t_0}} \sum_{t=t_l}^{t_0-1}, where $t_l$ is the first day when region l has confirmed cases.
b_{R}^* &= b_{R}- \sum_{(t,l) \in \Omega_{t_0}}  \left( {X_{l, t+1}^{R} - X_{l, t}^{R}} \right) + \sum_{(t,l) \in \Omega_{t_0}} {X_{l, t}^{I}}.
\end{aligned}
\end{equation*}
\raggedbottom



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{More on the Policy Search Algorithms}
\subsection{Constrained simultaneous perturbation stochastic approximation}\label{sec:SPSA}

When $J$ is large, Algorithm \ref{alg:grid} in the main paper can be computationally expensive. 
In general, a variety of optimization algorithms, such as Bayesian optimization and heuristic optimization algorithms, can be applied here. 
As an example, we provide a constrained simultaneous perturbation stochastic approximation (SPSA) algorithm  \cite{sadegh1997constrained} here. 
%  for more general settings
It is described in Algorithm \ref{alg:SPSA}. 
In SPSA, we need to specify two step size sequences $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}$, which  should satisfy $\sum_{k = 1}^{\infty} \zeta_k = \infty, \sum_{k = 1}^{\infty} \zeta_k^2 < \infty$ and $\xi_k = o(1)$ as $k$ goes to infinity. %? not uniform?
% In our experiments, we use $\zeta_k = \zeta / k^{\tau}$ and $\xi_k = \xi/k$, where $\zeta, \xi$  and $\tau \in (0.5,1]$ are  tuning parameters. 
Unlike traditional SPSA, for each candidate parameter $\vlam_t^k$, we run $M$ replications of Monte Carlo instead of only once and use the average to approximate the expected average utility. 
This is because that, in our setting, the sampling is relatively cheap and the potential loss of a sub-optimal policy can be quite severe. 
The operator $\mathbb{P}_{E_k}$ is the orthogonal projection onto  $E_k$ and it ensures the feasibility of policy evaluation under the constraints. 
Following \cite{sadegh1997constrained}, we define $E_k = \{\vlam: \lam_J + \xi_k\sqrt{J - 1} \le \lam_M, \lam_i + \xi_k\sqrt{J - 1} \le \lam_{i + 1} , \forall i \in \{1,\dots,J-1\} \}$. 
The direction is sampled from a distribution $\mathbb{G}$ of dimension $J-2$. 
The convergence of SPSA is guaranteed by our choice of $\zeta_k$.
In implementations, 
warm start can be used by setting $\vlam^1 = \vlam_{t_0 - 1}$ to further reduce the computational burden and 
multi-start random initialization can also be employed to remedy the non-convexity. 
% \hl{needs update Ek. already done in the code}
% Denote the feasible parameter region as $E = \{\vlam: 0 \le \lam_2 \le \dots \le \lam_{J} \le \lam_M\}$. 


\input{Algorithms/Algo_SPSA.tex}


\subsection{Deep Q-learning}\label{sec:supp-DQN}
When the global optimality is preferred, we can choose a general policy class and apply cutting-edge RL algorithms to solve the planning problem. 
In Algorithm \ref{alg:DQN}, we modify the deep-Q learning algorithm to take into consideration the learned uncertainty on $\vthe$.  
% used in our experiment. 
More details abou the standard DQN can be found in \cite{mnih2015human}. 


\input{Algorithms/DQN}




\subsection{Computational complexity}\label{sec:complexity}

In this section, we discuss the computational complexity of our policy search algorithm. 
We first consider a general form of the grid search algorithm presented in Algorithm \ref{alg:grid}. 
Suppose we have $J$ action levels, and recall we have $J - 1$ policy parameters $\lam_2, \dots, \lam_J$. 
Let the step size for searching $\lam_j$ be $\xi_j$ and the corresponding upper search bound be $U_j$, for $j = 2, \dots, J$. 
Define $\eta = max_{j \in \{2, \dots, J\}} (U_j / \xi_j)$. 
Assume that for each candidate policy, we run $M$ replications of rollouts.  
Using similar iteration schedule with Algorithm \ref{alg:grid} in the main paepr,
the computational complexity is easy to calculate as $O(M T \eta^{J - 1})$, where $T$ is the horizon. 
Then it is straightforward to show that the computational complexity of Algorithm 1 is $O(MB T \eta^{J - 1} + BKT)$, where $B$ is the number of candidate weights and $K$ is the number of Monte Carlo replications. 
Due to the importance of a stable optimization algorithm in our application, we choose to use this grid search algorithm in our experiment and recommend a large $M$. 
This is feasible when $J$ is not large, for example, $3$ or $5$. 
However, because its complexity is of exponential order with respect to $J$, when there are many actions available, we should choose other optimization algorithms such as Algorithm \ref{alg:SPSA}, with a large $M$ to reduce the variance from Monte Carlo rollouts. 
The algorithm is embarrassingly parallel. 
For the DQN-based method, the complicity is $B$ times of that of the standard deep-Q learning algorithm. 

\subsection{Hyper-parameters}
In this section, we describe the hyper-parameters used in our experiments. 
For the grid search algorithm, the number of rollout replications is set as $M = 100$. 
We run the grid search algorithm from coarse grids to finer grids to save computational cost. 
The schedule is listed in Table \ref{table:para}. 
In generally, the larger the search spaces and the smaller the step sizes, the better the performance will be. 
In consideration of the importance of this application and the relatively lightweight computation, in real application, we can choose the search spaces as large enough and step size as small enough. 
% $\lambda_M$ is another upper bound which indicates that, no matter

For DQN, in our experiment, we use a dense network of 5 layers, with 32 nodes per layer, to model the Q-function. 
The activation function is picked as relu and the optimizer is set as Adam. 
The learning rate is fixed as 0.0002 and the parameter for epsilon-greedy is set as $\epsilon = 0.1$. 
% max_epoch = 100


% &   $\beta_3$ 
\begin{table*}[t!]
\centering
    \caption{Search space and step sizes for the grid search in each round. $\lam^i_1$ and $\lam^i_2$ are the output from the $i$-th round.}
    \label{table:para}
    \begin{tabular}{lllllll}
\toprule
  round & $u_2$  &  $u_3$    & $U_2$  & 
  $U_3$ &   $\xi_2$ &   $\xi_3$  \\
\midrule
1 & 0& 300& 50& 0& 100& 200 \\
2 &  max(0, $\lam^1_1$ - 50)&  $\lam^1_1$ + 50& 5& $\lam^1_2$ - 200& $\lam^1_2$ + 200& 20 \\
3 &  max(0, $\lam^2_1$ - 5)&  $\lam^2_1$ + 5& 1& $\lam^2_2$ - 20& $\lam^2_2$ + 20& 4 \\
4 &  max(0, $\lam^3_1$ - 1)&  $\lam^3_1$ + 1& 0.25& $\lam^3_2$ - 4& $\lam^3_2$ + 4& 1 \\
5 &  max(0, $\lam^4_1$ - 0.25)&  $\lam^4_1$ + 0.25& 0.01& $\lam^4_2$ - 1& $\lam^4_2$ + 1& 0.2 \\
\bottomrule
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Details of the numerical experiments}

% In this section, we provide mores details of Section \ref{sec:numerical} and addtional numerical results. 

\subsection{More on the China COVID-19 dataset and hyper-parameters}\label{sec:supp-data}

We obtain the counts of cumulative confirmed cases $O_{l,t}^I$ from  \cite{China_Data} with irregular records imputed by the average of their neighbors.
The original mobility data collected from the online plateform Baidu Qianxi\footnote{http://qianxi.baidu.com} includes ${m_{l,t}^{20}}$, the mobility of people in city $l$ on day $t$ in  2020, and ${m_{l,t}^{19}}$, the value for the same date in 2019, aligned by the lunar calendar.  
We define $r_{l,t}=1- m_{l,t}^{20}/m_{l,t}^{19}$ to 
measure the  ratio of human mobility loss due to $A_{l,t}$. 
The fitted distributions for the intervention cost function are $C_2 \sim \mathcal{N}(0.368, 0.239^2)$ and 
$C_3 \sim \mathcal{N}(0.484, 0.181^2)$.
% C_3 rather than C_2
As for the action data, we collect the date ranges for different control measures claimed by Chinese local governments. 
The date ranges for action $1$ and $2$ as well as the starting dates for action $3$ are collected from \cite{wiki:action}. 
The ending dates for action $3$ are manually collected from the local government websites or their social media accounts. 
These data sources are all in Chinese. 
We use the estimates for SARS \cite{mkhatshwa2010modeling} to set the priors for the disease features, specifically, we set $\gamma \sim Beta(178.89, 2000)$ and $ \beta_1 \sim Gamma(517.41, 2000)$.
As for $\beta_2$ and $\beta_3$, similar with the assumptions in \cite{ferguson2020impact}, we assume the two measures reduce the infection rate by $80\%$ and $90\%$ respectively, and therefore use $\beta_2 \sim Gamma(103.48 , 2000)$ and $ \beta_3 \sim Gamma(51.74, 2000)$. 


% Since $X_{l,t}^R$ should be monotonically non-decreasing with respect to $t$ and there are some records violating this quality, we have substituted the peculiar records with mean values of their neighbors. 
% Figure \ref{fig:cost} shows the boxplot of the mobility loss ratio for different actions. 




\subsection{Validation of the simulation environment}\label{sec:supp_val}

We apply a leave-one-out cross-validation procedure to show that our simulation environment is close to the real data generation process. 
Specifically, for $l = 1, \dots, 6$, we follow the steps: 
\begin{enumerate}
    \item estimate the environmental parameter $\vthe$ as $\hat{\vthe}_l$, using all data  until day $61$ of cities in $\{1, \dots, 6\} \setminus \{l\}$.
    % day 10 = [2020-01-24]
    % day 61 = [2020-03-15]
    % day 120 = [2020-05-13]
    \item for city $l$, based on $\hat{\vthe}_l$, we predict its counts of the cumulative infected cases from day $12$ to day $120$, following the observed actions in the data. Denote the estimate for day $120$ as $\hat{X}^R_{120, l}.$ 
    % , t=10, 11,\cdots, 120$.
    \item calculate the approximation error by $\epsilon_{l} = |\hat{X}^R_{120, l} - O^I_{120,l}| / O^I_{120,l}$, where $O^I_{120,l}$ is the observed cumulative infected count for city $l$ until day $120$. 
\end{enumerate}

The average error ratio $\sum_{l = 1}^6 \epsilon_{l} / 6 = 0.18$  indicates that the environment is a relatively valid proxy for the real data generation process, 
and supports the fairness of our comparison with the behaviour policy. 

\subsection{Statistical significance of the policy evaluation results}

In Figure \ref{figure:Pareto} in the main paper, we compare  our algorithm with the other competing policies by 
the average costs following each policy. 
To examine the statistical significance of our results, we report the corresponding $95\%$ confidence interval for each average value in Figure \ref{figure:Paretosquare}. 
We can observe that our findings in Section \ref{sec:policy} are  statistically significant. 
The variance for the DQN-based method is slightly larger due to the limited computational resources, and we expect it will become stabler with more computation. 
Results for the other experiments are similar. 

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{figures/more_final_val.png}
% 	\caption{Validation result with the least RMSE, where $\mathcal{L}_i=\{$Beijing, Guangzhou, Shanghai$\}$ and $\mathcal{L}'_i=\{$Hefei, Nanjing, Tianjin$\}.$}\label{fig:cv3}
% \end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{figures/main_with_DQN_sd.png} 
% Figure1_supp_factor10
\caption{Cumulative epidemiological cost and economic cost  following different policies, averaged over $100$ replications. The closer to the left bottom corner, the better. With the shaded areas indicating the 95$\%$ confidence regions.}
\label{figure:Paretosquare}
\end{figure}

\subsection{Sample policies displayed in the demo}
In Figure \ref{fig:pareto_demo}, we apply the policy search algorithm in the threshold-based policy class, and zoom in to analyze three Pareto-optimal policies. 
Here, we give their policy parameters to provide more details. 
For policy A, B, and C, their $\vlam$ is $(0,0)^T$, $(0.26,  420)^T$, and $(245, 573)^T$, respectively. 
This explains their behaviour: policy A is a strict one and assigns level 3 whenever the algorithm believes there is any infectious individual; 
policy B is milder, and it typically imposes the level-2 action unless the spread is quite severe; policy C is much more loose. 


\section{Sensitivity analysis}\label{sec: supp-robust}

\subsection{Robustness against model missepcification}\label{sec: supp-robust-analysis}
In this section, we investigate the robustness of the proposed framework against potential model missepcification. 
We use a generalized Susceptible-Exposed-Infected-Removal model (SEIR) model instead of the GSIR model as the data generation model, and conduct a simulation study similar with the one in Section \ref{sec:numerical_policy}. 
% with the setting kept the same
The standard SEIR model is another commonly used compartmental model, which adds one additional exposed compartment to the SIR model. 
See Figure \ref{figure:SEIR} for an illustration and refer to \cite{tang2020review} for a detailed introduction. 

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{figures/SEIR.png} 
\caption{A diagram for the standard SEIR model.}
\label{figure:SEIR}
\end{figure}

We generalize the SEIR model in a similar with as the GSIR model, by including the action effects into consideration to set the infection rate $\beta$. The transition from the susceptible compartment to the exposed compartment is assumed to follow a binomial distribution with parameter $\alpha$. 
According to \cite{yang2020modified}, we set the incubation rate $\alpha$ as $1/7$. 
The other parameters are kept the same with Section \ref{sec:numerical_policy}. 
Since the exposed compartment is typically latent,  the number of individuals in this compartments on the beginning date can not be set based on the real data as the other compartments. 
For experiment purpose, we set the number to be the same with the number in the infectious compartment. 

The results are presented in Figure \ref{figure:Pareto_SEIR}. 
As expected, compared with results under the GSIR model, the performance of the  proposed method under this setting slightly deteriorates. 
However, in generally, the method still over-performs the other fixed policies, and also provides more options with a clear trade-off.  



\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{figures/SEIR_with_DQN.png} 
\caption{Simulated results when the true data generation model is the generalized SEIR model. Cumulative epidemiological cost and economic cost  following different policies, averaged over $100$ replications.}
\label{figure:Pareto_SEIR}
\end{figure}


\subsection{Hyper-parameter sensitivity analysis}\label{sec:sensitivity}
Our framework requires selecting several hyper-parameters according to domain knowledge, and our choices in the experiments largely follow the practice in the early period of the COVID-19 outbreak and are listed in Section \ref{sec:supp-data}. 
On one hand, at the beginning of an pandemic we have to rely on some priors to make decision; and on the other hand, in this section we use numerical experiments to evaluate the robustness of our algorithm to these hyper-parameters. 
The setting is kept the same with Section \ref{sec:numerical_policy}, except for that we only run 25 replications for the proposed algorithm to save computation. 
We present results for the threshold-based policy class. 
Results for the DQN-based methods are similar and omitted. 

In Figure \ref{figure:robust_lag}, we report the results with $D = 7, 8, 9, 10, 11$. 
It can be seen that, although the results varies a little, the algorithm generally still outperform the competing policies, and our findings in Section \ref{sec:numerical_policy} still hold. 

% \begin{figure}[h!]
% \centering
% \includegraphics[width=.45\textwidth]{figures/robust_lag.png} 
% \caption{Robust analysis results for the hyper-parameter $D$.}
% \label{figure:robust_lag}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width=.45\textwidth]{figures/robust_effect.png} 
% \caption{Robust analysis results for the hyper-parameter $\mu_1$ and $\mu_2$.}
% \label{figure:robust_effect}
% \end{figure}


\begin{figure*}[t]
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=.8\textwidth]{figures/robust_lag.png} 
\caption{Robust analysis results for the hyper-parameter $D$.}
\label{figure:robust_lag}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=.8\textwidth]{figures/robust_effect.png} 
\caption{Robust analysis results for the hyper-parameter $\mu_1$ and $\mu_2$.}
\label{figure:robust_effect}
\end{subfigure}
\caption{Hyper-parameter sensitivity analysis}
\label{fig:sensitivity}
\end{figure*}



Similarly, we report the robustness analysis results for the treatment effects $\mu_2$ and $\mu_3$ In Figure \ref{figure:robust_effect}. 
Recall that we define $\mu_j = \beta_j / \beta_1$ and use it to set the prior for $\beta_i$. 
In our experiment, we use $\mu_2 = 0.2$ and $\mu_3 = 0.1$. 
In this analysis, we present results for $\{(\mu_2, \mu_3): \mu_3 \in \{0.05, 0.1, 0.15, 0.2\}
, \mu_2 - \mu_3 \in \{0.05, 0.1, 0.15, 0.2\} )\}$. 
These prior parameters turn out have little important in the long run, because their effects get washed out quickly by the observed data. 
The findings for the other prior parameters are similar. 

\break

\bibliography{bib}
\bibliographystyle{plain}
	
\end{document}


==> COVID_KDD (Camara Ready) [Arxiv]/Archive/supp_sty.tex <==

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
% \usepackage{neurips_2020}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2020}

% to avoid loading the natbib package, add option nonatbib:
% \usepackage{Mis/neurips_2020}
\usepackage{Mis/aaai21}
\input{Mis/packages}


\usepackage{amsmath}
\usepackage{graphicx}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{algorithm,algpseudocode,enumerate}
\usepackage{bm}
\usepackage{hyperref}       % hyperlinks
\usepackage{xr-hyper}
% \usepackage{pdfpages}
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\myexternaldocument{0_MAIN}
\newtheorem{lemma}{Lemma}[section]

==> COVID_KDD (Camara Ready) [Arxiv]/sec_SPCA.tex <==
\subsection{Constrained simultaneous perturbation stochastic approximation}\label{sec:SPSA}

When $J$ is large, Algorithm \ref{alg:grid} in the main paper can be computationally expensive. 
In general, a variety of optimization algorithms, such as Bayesian optimization and heuristic optimization algorithms, can be applied here. 
As an example, we provide a constrained simultaneous perturbation stochastic approximation (SPSA) algorithm  \cite{sadegh1997constrained} here. 
%  for more general settings
It is described in Algorithm \ref{alg:SPSA}. 
In SPSA, we need to specify two step size sequences $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}$, which  should satisfy $\sum_{k = 1}^{\infty} \zeta_k = \infty, \sum_{k = 1}^{\infty} \zeta_k^2 < \infty$ and $\xi_k = o(1)$ as $k$ goes to infinity. %? not uniform?
% In our experiments, we use $\zeta_k = \zeta / k^{\tau}$ and $\xi_k = \xi/k$, where $\zeta, \xi$  and $\tau \in (0.5,1]$ are  tuning parameters. 
Unlike traditional SPSA, for each candidate parameter $\vlam_t^k$, we run $M$ replications of Monte Carlo instead of only once and use the average to approximate the expected average utility. 
This is because that, in our setting, the sampling is relatively cheap and the potential loss of a sub-optimal policy can be quite severe. 
The operator $\mathbb{P}_{E_k}$ is the orthogonal projection onto  $E_k$ and it ensures the feasibility of policy evaluation under the constraints. 
Following \cite{sadegh1997constrained}, we define $E_k = \{\vlam: \lam_J + \xi_k\sqrt{J - 1} \le \lam_M, \lam_i + \xi_k\sqrt{J - 1} \le \lam_{i + 1} , \forall i \in \{1,\dots,J-1\} \}$. 
The direction is sampled from a distribution $\mathbb{G}$ of dimension $J-2$. 
The convergence of SPSA is guaranteed by our choice of $\zeta_k$.
In implementations, 
warm start can be used by setting $\vlam^1 = \vlam_{t_0 - 1}$ to further reduce the computational burden and 
multi-start random initialization can also be employed to remedy the non-convexity. 
% \hl{needs update Ek. already done in the code}
% Denote the feasible parameter region as $E = \{\vlam: 0 \le \lam_2 \le \dots \le \lam_{J} \le \lam_M\}$. 


\input{Algorithms/Algo_SPSA.tex}


==> COVID_KDD (Camara Ready) [Arxiv]/sec_comp_complexity.tex <==
\subsection{Computational complexity}\label{sec:complexity}

In this section, we discuss the computational complexity of our policy search algorithm. 
We first consider a general form of the grid search algorithm presented in Algorithm \ref{alg:grid}. 
Suppose we have $J$ action levels, and recall we have $J - 1$ policy parameters $\lam_2, \dots, \lam_J$. 
Let the step size for searching $\lam_j$ be $\xi_j$ and the corresponding upper search bound be $U_j$, for $j = 2, \dots, J$. 
Define $\eta = max_{j \in \{2, \dots, J\}} (U_j / \xi_j)$. 
Assume that for each candidate policy, we run $M$ replications of rollouts.  
Using similar iteration schedule with Algorithm \ref{alg:grid} in the main paepr,
the computational complexity is easy to calculate as $O(M T \eta^{J - 1})$, where $T$ is the horizon. 
Then it is straightforward to show that the computational complexity of Algorithm 1 is $O(MB T \eta^{J - 1} + BKT)$, where $B$ is the number of candidate weights and $K$ is the number of Monte Carlo replications. 
Due to the importance of a stable optimization algorithm in our application, we choose to use this grid search algorithm in our experiment and recommend a large $M$. 
This is feasible when $J$ is not large, for example, $3$ or $5$. 
However, because its complexity is of exponential order with respect to $J$, when there are many actions available, we should choose other optimization algorithms such as Algorithm \ref{alg:SPSA}, with a large $M$ to reduce the variance from Monte Carlo rollouts. 
The algorithm is embarrassingly parallel. 
For the DQN-based method, the complicity is $B$ times of that of the standard deep-Q learning algorithm. 


==> COVID_KDD (Camara Ready) [Arxiv]/sec_std.tex <==
\subsection{Statistical significance of the policy evaluation results}

In Figure \ref{figure:Pareto} in the main paper, we compare  our algorithm with the other competing policies by 
the average costs following each policy. 
To examine the statistical significance of our results, we report the corresponding $95\%$ confidence interval for each average value in Figure \ref{figure:Paretosquare}. 
We can observe that our findings in Section \ref{sec:policy} are  statistically significant. 
The variance for the DQN-based method is slightly larger due to the limited computational resources, and we expect it will become stabler with more computation. 
Results for the other experiments are similar. 

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{figures/more_final_val.png}
% 	\caption{Validation result with the least RMSE, where $\mathcal{L}_i=\{$Beijing, Guangzhou, Shanghai$\}$ and $\mathcal{L}'_i=\{$Hefei, Nanjing, Tianjin$\}.$}\label{fig:cv3}
% \end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth, height=.5\textwidth]{figures/main_with_DQN_sd.png} 
% Figure1_supp_factor10
\caption{Cumulative epidemiological cost and economic cost  following different policies, averaged over $100$ replications. The closer to the left bottom corner, the better. With the shaded areas indicating the 95$\%$ confidence regions.}
\label{figure:Paretosquare}
\end{figure}


==> sec_SPCA.tex <==
\subsection{Constrained simultaneous perturbation stochastic approximation}\label{sec:SPSA}

When $J$ is large, Algorithm \ref{alg:grid} in the main paper can be computationally expensive. 
In general, a variety of optimization algorithms, such as Bayesian optimization and heuristic optimization algorithms, can be applied here. 
As an example, we provide a constrained simultaneous perturbation stochastic approximation (SPSA) algorithm  \cite{sadegh1997constrained} here. 
%  for more general settings
It is described in Algorithm \ref{alg:SPSA}. 
In SPSA, we need to specify two step size sequences $\{\zeta_k\}_{k\ge 1}$ and $\{\xi_k\}_{k\ge 1}$, which  should satisfy $\sum_{k = 1}^{\infty} \zeta_k = \infty, \sum_{k = 1}^{\infty} \zeta_k^2 < \infty$ and $\xi_k = o(1)$ as $k$ goes to infinity. %? not uniform?
% In our experiments, we use $\zeta_k = \zeta / k^{\tau}$ and $\xi_k = \xi/k$, where $\zeta, \xi$  and $\tau \in (0.5,1]$ are  tuning parameters. 
Unlike traditional SPSA, for each candidate parameter $\vlam_t^k$, we run $M$ replications of Monte Carlo instead of only once and use the average to approximate the expected average utility. 
This is because that, in our setting, the sampling is relatively cheap and the potential loss of a sub-optimal policy can be quite severe. 
The operator $\mathbb{P}_{E_k}$ is the orthogonal projection onto  $E_k$ and it ensures the feasibility of policy evaluation under the constraints. 
Following \cite{sadegh1997constrained}, we define $E_k = \{\vlam: \lam_J + \xi_k\sqrt{J - 1} \le \lam_M, \lam_i + \xi_k\sqrt{J - 1} \le \lam_{i + 1} , \forall i \in \{1,\dots,J-1\} \}$. 
The direction is sampled from a distribution $\mathbb{G}$ of dimension $J-2$. 
The convergence of SPSA is guaranteed by our choice of $\zeta_k$.
In implementations, 
warm start can be used by setting $\vlam^1 = \vlam_{t_0 - 1}$ to further reduce the computational burden and 
multi-start random initialization can also be employed to remedy the non-convexity. 
% \hl{needs update Ek. already done in the code}
% Denote the feasible parameter region as $E = \{\vlam: 0 \le \lam_2 \le \dots \le \lam_{J} \le \lam_M\}$. 


\input{Algorithms/Algo_SPSA.tex}


==> sec_comp_complexity.tex <==
\subsection{Computational complexity}\label{sec:complexity}

In this section, we discuss the computational complexity of our policy search algorithm. 
We first consider a general form of the grid search algorithm presented in Algorithm \ref{alg:grid}. 
Suppose we have $J$ action levels, and recall we have $J - 1$ policy parameters $\lam_2, \dots, \lam_J$. 
Let the step size for searching $\lam_j$ be $\xi_j$ and the corresponding upper search bound be $U_j$, for $j = 2, \dots, J$. 
Define $\eta = max_{j \in \{2, \dots, J\}} (U_j / \xi_j)$. 
Assume that for each candidate policy, we run $M$ replications of rollouts.  
Using similar iteration schedule with Algorithm \ref{alg:grid} in the main paepr,
the computational complexity is easy to calculate as $O(M T \eta^{J - 1})$, where $T$ is the horizon. 
Then it is straightforward to show that the computational complexity of Algorithm 1 is $O(MB T \eta^{J - 1} + BKT)$, where $B$ is the number of candidate weights and $K$ is the number of Monte Carlo replications. 
Due to the importance of a stable optimization algorithm in our application, we choose to use this grid search algorithm in our experiment and recommend a large $M$. 
This is feasible when $J$ is not large, for example, $3$ or $5$. 
However, because its complexity is of exponential order with respect to $J$, when there are many actions available, we should choose other optimization algorithms such as Algorithm \ref{alg:SPSA}, with a large $M$ to reduce the variance from Monte Carlo rollouts. 
The algorithm is embarrassingly parallel. 
For the DQN-based method, the complicity is $B$ times of that of the standard deep-Q learning algorithm. 


==> sec_std.tex <==
\subsection{Statistical significance of the policy evaluation results}

In Figure \ref{figure:Pareto} in the main paper, we compare  our algorithm with the other competing policies by 
the average costs following each policy. 
To examine the statistical significance of our results, we report the corresponding $95\%$ confidence interval for each average value in Figure \ref{figure:Paretosquare}. 
We can observe that our findings in Section \ref{sec:policy} are  statistically significant. 
The variance for the DQN-based method is slightly larger due to the limited computational resources, and we expect it will become stabler with more computation. 
Results for the other experiments are similar. 

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{figures/more_final_val.png}
% 	\caption{Validation result with the least RMSE, where $\mathcal{L}_i=\{$Beijing, Guangzhou, Shanghai$\}$ and $\mathcal{L}'_i=\{$Hefei, Nanjing, Tianjin$\}.$}\label{fig:cv3}
% \end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth, height=.5\textwidth]{figures/main_with_DQN_sd.png} 
% Figure1_supp_factor10
\caption{Cumulative epidemiological cost and economic cost  following different policies, averaged over $100$ replications. The closer to the left bottom corner, the better. With the shaded areas indicating the 95$\%$ confidence regions.}
\label{figure:Paretosquare}
\end{figure}

